Estimating the Sizes of Binary Error-Correcting Constrained Codes

In this paper, we study binary constrained codes that are resilient to bit-flip errors and erasures. In our first approach, we compute the sizes of constrained subcodes of linear codes. Since there exist well-known linear codes that achieve vanishing probabilities of error over the binary symmetric channel (which causes bit-flip errors) and the binary erasure channel, constrained subcodes of such linear codes are also resilient to random bit-flip errors and erasures. We employ a simple identity from the Fourier analysis of Boolean functions, which transforms the problem of counting constrained codewords of linear codes to a question about the structure of the dual code. We illustrate the utility of our method in providing explicit values or efficient algorithms for our counting problem, by showing that the Fourier transform of the indicator function of the constraint is computable, for different constraints. Our second approach is to obtain good upper bounds, using an extension of Delsarte's linear program (LP), on the largest sizes of constrained codes that can correct a fixed number of combinatorial errors or erasures. We observe that the numerical values of our LP-based upper bounds beat the generalized sphere packing bounds of Fazeli, Vardy, and Yaakobi (2015).

==> Preliminaries-fourier.tex <==
\label{sec:preliminaries}
\subsection{Notation}
\label{sec:notation}
Given integers $a, b$, we use the notation $[a:b]$ to denote the set $\{a,a+1,\ldots,b\}$, for $a\leq b$. We use $[n]$ as shorthand for $[1:n]$. For a vector $\mathbf{a}\in \{0,1\}^n$, we denote by $w(\mathbf{a})$ its Hamming weight (or, simply, weight), i.e., $w(\mathbf{a})$ is the number of ones present in $\mathbf{a}$, and we use the notation supp$(\mathbf{a})$ to denote the set of coordinates $\{i\in[n]:\ a_i = 1\}$. We say that a length-$n$ vector $\mathbf{a}$ is supported on $S\subseteq [n]$, if supp$(\mathbf{a})\subseteq S$. Further, given a length-$n$ vector $\mathbf{a}$, let $a_i^j$ denote the vector $(a_k:\ i\leq k\leq j)$, for $j\leq n$. Given a length $n$, we let $\mathbf{B}_n(i)$ denote the binary representation of $0\leq i\leq 2^n-1$. The subscript `$n$' will be dropped when evident from the context. Further, for $\mathbf{z}\in \{0,1\}^n$, we define $w_\mathbf{z}(\mathbf{a})$ to be the number of ones in $\mathbf{a}$, in the positions in supp$(\mathbf{z})$. For $r\in \{0,1\}$, we define the vector $r^m$ to be the length-$m$ vector all of whose symbols equal $r$. Further, given two binary vectors $\mathbf{a} = (a_1,\ldots,a_n)$ and $\mathbf{b} = (b_1,\ldots,b_n)$, their dot product $\mathbf{a}\cdot \mathbf{b}$ equals $\sum_{i=1}^n a_i b_i$, and we denote their concatenation by $\mathbf{a}\mathbf{b}$ or $(\mathbf{a}\mid \mathbf{b})$. For an $m\times n$ matrix $M$, we use the notation $M[i]$ to denote its $i^{\text{th}}$ column, for $i\in [n]$, and $M(j)$ to denote its $j^{\text{th}}$ row, for $j\in [m]$. For a given real number $r\in \mathbb{R}$, we define $\left \lfloor r\right \rfloor$ and $\left \lceil r\right \rceil$ to be, respectively, the largest integer less than or equal to $r$, and the smallest integer larger than or equal to $r$. For a set $P\subseteq \{0,1\}^n$, we use the notation $$\mathds{1}_{P}(\mathbf{x}) = \begin{cases}1,\ \text{if $\mathbf{x}\in P$},\\0,\ \text{otherwise.}\end{cases}$$
%Moreover, for a real $x$, we define the function
%\[
%\text{sgn}(x) := \begin{cases}
%	-1,\ \text{if $x<0$},\\
%	0,\ \text{if $x=0$},\\
%	+1,\ \text{otherwise}.
%\end{cases}
%\]
\subsection{Block Codes and Constrained Sequences}
We recall the following definitions of block codes and linear codes over $\mathbb{F}_2$ (see, for example, Chapters 1 and 2 of \cite{roth_coding_theory}).

\begin{definition}
	An $(n,M)$ block code $\mathcal{C}$ over $\mathbb{F}_2$ is a nonempty subset of $\mathbb{F}_2^n$, with $|\mathcal{C}| = M$. The rate of the block code $\mathcal{C}$ is given by
	\[
	\text{rate}(\mathcal{C}) := \frac{\log_2 M}{n}.
	\]
\end{definition}
Moreover, given a sequence of block codes $\{\mathcal{C}^{(n)}\}_{n\geq 1}$, if it holds that rate$(\mathcal{C}^{(n)})\xrightarrow{n\to \infty} R$, for some $R\in [0,1]$, then we say that $\{\mathcal{C}^{(n)}\}_{n\geq 1}$ is of rate $R$.
\begin{definition}
	An $[n,k]$ linear code $\mathcal{C}$ over $\mathbb{F}_2$ is an $(n,2^k)$ block code that is a subspace of $\mathbb{F}_2^n$.
\end{definition}
A constraint is represented by a set $\mathcal{A}\subseteq \{0,1\}^n$ of binary words. We call the sequences in $\mathcal{A}$ as \emph{constrained} sequences. Given such a collection of constrained sequences of blocklength $n$, the noiseless capacity (see Chapter 3 of \cite{Roth}) of the constraint is defined as
\[
C_0(\mathcal{A}):= \lim_{n\to \infty} \frac{\log_2 |\mathcal{A}|}{n},
\] 
where the limit in the expression above exists, by subadditivity arguments.
%%Consider now a set $S^{(n)}$ of length-$n$ binary words that satisfy the $(d,\infty)$-RLL constraint. We recall the following definition (see, for example, Chapter 3 of \cite{Roth}):
%%\begin{definition}
%%	The noiseless capacity $C_0^{(d)}$ of the $(d,\infty)$-RLL constraint is defined as
%%	\[
%%	C_0^{(d)}:= \lim_{n\to \infty} \frac{\log_2\left\lvert S_{(d,\infty)}^{(n)}\right \rvert}{n} = \inf_n \frac{\log_2\left\lvert S_{(d,\infty)}^{(n)}\right \rvert}{n},
%%	\]
%%	where the last equality follows from the subadditivity of the sequence $\left(\log_2\left\lvert S_{(d,\infty)}^{(n)}\right\rvert\right)_{n\geq 1}$. 
%\end{definition}
\subsection{Fourier Expansion of Boolean Functions}
\label{sec:fourierprelim}
Consider functions $f: \{0,1\}^n\to \mathbb{R}$, mapping $\mathbf{x} = (x_1,\ldots,x_n) \in \{0,1\}^n$ to $f(\mathbf{x})\in \mathbb{R}$. If the range of $f$ is $\{0,1\}$, then $f$ is called a Boolean function.  Now, given any function $f: \{0,1\}^n\to \mathbb{R}$ and a vector $\mathbf{s} = (s_1,\ldots,s_n)\in \{0,1\}^n$, we define the Fourier coefficient of $f$ at $\mathbf{s}$ as
\[
\widehat{f}(\mathbf{s}):= \frac{1}{2^n}\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x})\cdot (-1)^{\mathbf{x}\cdot \mathbf{s}}.
\]
The function $\widehat{f}$ is known as the Fourier transform (sometimes called the Hadamard transform) of $f$. Moreover, the functions $\left(\chi_{\mathbf{s}}: \mathbf{s}\in \{0,1\}^n\right)$, where $\chi_{\mathbf{s}}(\mathbf{x}):=(-1)^{\mathbf{x}\cdot \mathbf{s}}$, form a basis for the vector space $V$ of functions $f: \{0,1\}^n\to \mathbb{R}$. If we define an inner product $\langle \cdot, \cdot \rangle$ over the vector space $V$, as follows:
\[
\langle f,g \rangle := \frac{1}{2^n}\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x}) g(\mathbf{x}),
\]
for functions $f,g \in V$, we also have that the basis functions $\left(\chi_{\mathbf{s}}: \mathbf{s}\in \{0,1\}^n\right)$ are orthonormal, in that
\[
\langle \chi_{\mathbf{s}},\chi_{\mathbf{s}^\prime} \rangle = 
\begin{cases}
	1,\ \text{if $\mathbf{s} = \mathbf{s}^\prime$},\\
	0,\ \text{otherwise.}
\end{cases}
\]
The above discussion leads us to the following well-known theorem:
\begin{theorem}[Theorem 1.1 in \cite{ryanodonnell}]
	Every function $f: \{0,1\}^n\to \mathbb{R}$ can be uniquely expressed as its Fourier expansion
	\[
	f(\mathbf{x}) = \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{f}(\mathbf{s})\cdot (-1)^{\mathbf{x}\cdot \mathbf{s}}.
	\]
\end{theorem}
For more details on the Fourier analysis of Boolean functions, we refer the reader to \cite{ryanodonnell}. In our paper, we shall make use of Plancherel's Theorem from Fourier analysis, which is recalled below, without proof.
\begin{theorem}[Plancherel's Theorem]
	For any $f,g \in \{0,1\}^n\to \mathbb{R}$, we have that
	\[
	\langle f,g \rangle = \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{f}(\mathbf{s})\widehat{g}(\mathbf{s}).
	\]
\end{theorem}
\subsection{Key Ideas}
\label{sec:prelim}
Consider an $[n,k]$ linear code $\mathcal{C}$. Suppose that we are interested in computing the number of codewords $\mathbf{c}\in \mathcal{C}$ each of which satisfies a certain property, which we call a constraint (for background on constrained sequences and constrained coding, we refer the reader to \cite{Roth}). Let $\mathcal{A}\subseteq \{0,1\}^n$ denote the set of length-$n$ words that respect the constraint. Note that we make no further assumption about the constraint (such as it being finite-type, irreducible, etc.). We let $N(\mathcal{C};\mathcal{A})$ denote the number of such constrained codewords in $\mathcal{C}$. We can then write
\begin{align}
	\label{eq:countC}
	N(\mathcal{C};\mathcal{A}) &= \sum_{\mathbf{c}\in \mathcal{C}} \mathds{1}_{\mathcal{A}}(\mathbf{c}).
\end{align}
%where for a set $P$, we use the notation $$\mathds{1}_{P}(\mathbf{x}) = \begin{cases}1,\ \text{if $\mathbf{x}\in P$},\\0,\ \text{otherwise.}\end{cases}$$ 
Observe that the summation in \eqref{eq:countC} is over a set of size $2^k$, which could be quite large, especially when $k>n/2$. Our interest is in obtaining insight into the summation above, by employing a simple trick from the Fourier expansions of Boolean functions. 

Our first observation is summarized below as a theorem. For a linear code $\mathcal{C}$, we denote its dual code by $\mathcal{C}^{\perp}$.

\begin{theorem}
	\label{thm:lincount}
	Given a linear code $\mathcal{C}$ of blocklength $n$ and a set $\mathcal{A}\subseteq \{0,1\}^n$, we have that
	\[
	N(\mathcal{C};\mathcal{A}) = \left\lvert \mathcal{C}\right\rvert \cdot \sum_{\mathbf{s}\in \mathcal{C}^{\perp}} \widehat{\mathds{1}_\mathcal{A}}(\mathbf{s}).
	\]
\end{theorem}
\begin{proof}
	The proof is a straightforward application of Plancherel's Theorem. Observe that
	\begin{align}
	N(\mathcal{C};\mathcal{A}) &= \sum_{\mathbf{c}\in \mathcal{C}} \mathds{1}_{\mathcal{A}}(\mathbf{c}) \notag\\
	&= \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_{\mathcal{A}}(\mathbf{x})\cdot \mathds{1}_{\mathcal{C}}(\mathbf{x}) \notag \\
	&= 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s})\cdot \widehat{\mathds{1}_{\mathcal{C}}}(\mathbf{s}) \label{eq:inter1}.
	\end{align}
Now, we claim that 
\begin{equation}
	\label{eq:Ccoeff}
\widehat{\mathds{1}_{\mathcal{C}}}(\mathbf{s}) = \begin{cases}
	\frac{\left\lvert \mathcal{C} \right\rvert}{2^n},\ \text{if $\mathbf{s}\in \mathcal{C}^\perp$},\\
	0,\ \text{otherwise}.
\end{cases}
\end{equation}
To prove the above claim, recall that
\begin{align*}
	\widehat{\mathds{1}_{\mathcal{C}}}(\mathbf{s}) = \frac{1}{2^n}\sum_{\mathbf{x}\in \{0,1\}^n}\mathds{1}_{\mathcal{C}}(\mathbf{x})\cdot (-1)^{\mathbf{x}\cdot \mathbf{s}}.
\end{align*}

If $\mathbf{s}\in \mathcal{C}^\perp$, it holds that $\mathbf{x}\cdot \mathbf{s} = 0$, for all $\mathbf{x}\in \mathcal{C}$. Hence, in this case, we have that $\widehat{\mathds{1}_{\mathcal{C}}}(\mathbf{s}) = 	\frac{\left\lvert \mathcal{C} \right\rvert}{2^n}$. 

If $\mathbf{s}\notin \mathcal{C}^\perp$, this means that there is some $\mathbf{x}^\star \in \mathcal{C}$ such that $\mathbf{x}^\star\cdot \mathbf{s} = 1$. Further, it is true that $\mathbf{0}\cdot \mathbf{s} = 0$, with $\mathbf{0}\in \mathcal{C}$, since $\mathcal{C}$ is a linear code. Hence, to any $\mathbf{c}\in \mathcal{C}$ such that $\mathbf{c}\cdot \mathbf{s} = 0$, we can uniquely map the codeword $\mathbf{c}+\mathbf{x}^\star$ (where the summation is over $\mathbb{F}_2^n$), with the property that $\left(\mathbf{c}+\mathbf{x}^\star\right)\cdot \mathbf{s} = 1$. Since this map is bijective, we obtain that the number of codewords $\mathbf{x}\in \mathcal{C}$ such that $(-1)^{\mathbf{x}\cdot \mathbf{s}} = 1$, equals the number of codewords $\mathbf{x}\in \mathcal{C}$ such that $(-1)^{\mathbf{x}\cdot \mathbf{s}} = -1$, for $\mathbf{s}\notin \mathcal{C}^\perp$. Therefore, we get that in this case, $\widehat{\mathds{1}_{\mathcal{C}}}(\mathbf{s}) = 0$.

Plugging \eqref{eq:Ccoeff} back in \eqref{eq:inter1}, we see that
\begin{align*}
	N(\mathcal{C};\mathcal{A})&= \left \lvert \mathcal{C}\right\rvert \cdot \sum_{\mathbf{s}\in \mathcal{C}^\perp} \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s}).
\end{align*}
\end{proof}

Theorem \ref{thm:lincount} provides an alternative approach to addressing our problem of counting constrained codewords in linear codes. In particular, note that if $\mathcal{C}$ had large dimension, i.e., if $k>n/2$, then, it is computationally less intensive to calculate the number of constrained codewords using Theorem \ref{thm:lincount}, provided we knew the Fourier coefficients $\widehat{\mathds{1}_\mathcal{A}}(\mathbf{s})$, since $\text{dim}\left(\mathcal{C}^\perp\right) = n-k<n/2$, in this case. Additionally, if the structure of the Fourier coefficients is simple to handle, we could also use Theorem \ref{thm:lincount} to construct linear codes that have a large (or small) number of constrained codewords, or to obtain estimates of the number of constrained codewords in a fixed linear code. In the rest of the paper, we shall study various examples of constraints, which in turn correspond to sets $\mathcal{A}$, whose Fourier coefficients $\widehat{\mathds{1}_\mathcal{A}}(\mathbf{s})$ are computable either analytically or numerically.

Next, suppose that we are interested in computing the weight distribution of words in $\{0,1\}^n$ that lie in a (constrained) set $\mathcal{A}\subseteq \{0,1\}^n$. Let $a_{i,\mathcal{A}}$ denote the number of constrained words of weight $i\in [0:n]$ and recall the definition of the $i^\text{th}$-Krawtchouk polynomial $K_i^{(n)}$, for a given blocklength $n$, where $K_i^{(n)}(z) = \sum_{\ell=0}^{i} (-1)^\ell {z\choose \ell} {n-z\choose i-\ell}$. We also use the notation $W_i:=\{\mathbf{x}\in \{0,1\}^n: w(\mathbf{x}) = i\}$. The following theorem then holds true:

\begin{theorem}
	\label{thm:wtcount}
	The weight distribution of sequences that lie in a set $\mathcal{A}\subseteq \{0,1\}^n$ obeys
	\[
	a_{i,\mathcal{A}} = \sum_{j=0}^n K_i^{(n)}(j)\cdot \sum_{\mathbf{s}:\ w(\mathbf{s}) = j} \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s}),\quad i\in [0:n].
	\]
\end{theorem}
\begin{proof}
	The proof is again a simple application of Plancherel's Theorem. Observe that
	\begin{align}
		a_{i,\mathcal{A}} &\stackrel{}{=} \sum_{\mathbf{x}\in \mathcal{A}} \mathds{1}_{W_i}(\mathbf{x}) \notag\\
		&= \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_{W_i}(\mathbf{x})\cdot \mathds{1}_{\mathcal{A}}(\mathbf{x})  \notag \\
		&= 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\mathds{1}_{W_i}}(\mathbf{s})\cdot \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s})  \label{eq:inter2}.
	\end{align}
%where in (a) we use the notation $W_i:=\{\mathbf{x}\in \{0,1\}^n: w(\mathbf{x}) = i\}$. 
We now recall the well-known proof of the fact that  $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}) = K_i(w(\mathbf{s}))$ (see Chapter 5 in \cite{mws} for more details on Krawtchouk polynomials). Note that
\begin{align*}
	2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s})  = \sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i} (-1)^{\mathbf{x}\cdot \mathbf{s}}.
\end{align*}
Now, the summation on the right side depends only on the weight $w(\mathbf{s})$, i.e., for any permutation of coordinates $\pi: \{0,1\}^n\to \{0,1\}^n$, it holds that
\begin{align*}
\sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i}	(-1)^{\mathbf{x}\cdot \pi(\mathbf{s})} &= \sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i}  (-1)^{\pi(\mathbf{x})\cdot \pi(\mathbf{s})}\\
&= \sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i} (-1)^{\mathbf{x}\cdot \mathbf{s}}.
\end{align*}
In other words, we have that $\widehat{\mathds{1}_{W_i}}(\mathbf{s}) = \widehat{\mathds{1}_{W_i}}(\pi(\mathbf{s}))$. Hence, for $\mathbf{s}$ such that $w(\mathbf{s}) = j$, it suffices that we calculate $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}^\star)$, where $\mathbf{s}^\star = (s_1^\star,\ldots,s_n^\star)$ is such that $s_1^\star = \ldots = s_j^\star = 1$ and $s_{j+1}^\star=\ldots=s_n^\star = 0$. By a direct computation, it can be checked that $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}^\star) = \sum_{\ell=0}^{i} (-1)^\ell {j\choose \ell} {n-j\choose i-\ell} = 2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s})$. Plugging this back into \eqref{eq:inter2} and simplifying, we obtain the expression in the theorem.
\end{proof}
As before, Theorem \ref{thm:wtcount} implies that if the Fourier coefficients $\widehat{\mathds{1}_\mathcal{A}}(\mathbf{s})$ (or, the sum of Fourier coefficients at a fixed weight $\sum_{\mathbf{s}:\ w(\mathbf{s}) = j} \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s})$) were available to us, we can easily compute the number of constrained words of a given weight.

In the rest of the paper, we shall look at specific examples of constraints and apply the above theorems. In particular, as recurring motifs, we shall consider the $[2^m-1,2^m-1-m]$ binary Hamming code, for $m\geq 1$ and the binary Reed-Muller codes. Since the constraints we work with are sensitive to the ordering of coordinates of the code, in the sense that a permutation of the coordinates can transform a codeword that does not satisfy the constraint into one that does, we shall first fix a canonical ordering of coordinates for the codes that we analyze. For the binary Hamming code, we assume that a parity-check matrix $H_{\text{Ham}}$ is such that $H_{\text{Ham}}[i] = \mathbf{B}_m(i)$, for $1\leq i\leq 2^m-1$.

Note that the Reed-Muller (RM) family of codes are codes of potentially large blocklength. For $m\geq 1$ and $r\leq m$, the $r^\text{th}$-order binary Reed-Muller code RM$(m,r)$ is the set of binary vectors obtained as evaluations of multilinear Boolean polynomials $f(x_1,\ldots,x_m)$, in the variables $x_1,\ldots,x_m$, of maximum degree $r$, on points of the unit hypercube (see Chapter 13 of \cite{mws} for more information on Reed-Muller codes). We use the convention that the coordinates of RM$(m,r)$ are written as binary $m$-tuples that are ordered according to the standard lexicographic ordering, i.e., the $i^{\text{th}}$ coordinate from the start is the $m$-tuple $\mathbf{B}_m(i-1)$, for $1\leq i\leq 2^m$. We thus have that the blocklength of RM$(m,r)$ is $n=2^m$ and dim$(\text{RM}(m,r)) = \sum_{i=0}^r {m\choose i}=:{m\choose \leq r}$.

==> Preliminaries.tex <==
\label{sec:preliminaries}
\subsection{Notation}
\label{sec:notation}
Given integers $a, b$, we use the notation $[a:b]$ to denote the set $\{a,a+1,\ldots,b\}$, for $a\leq b$. We use $[n]$ as shorthand for $[1:n]$. For a vector $\mathbf{a}\in \{0,1\}^n$, we denote by $w(\mathbf{a})$ its Hamming weight (or, simply, weight), i.e., $w(\mathbf{a})$ is the number of ones present in $\mathbf{a}$. %and we use the notation supp$(\mathbf{a})$ to denote the set of coordinates $\{i\in[n]:\ a_i = 1\}$. We say that a length-$n$ vector $\mathbf{a}$ is supported on $S\subseteq [n]$ if supp$(\mathbf{a})\subseteq S$. 
Given a pair of vectors $\mathbf{a},\mathbf{b} \in \mathbb{R}^n$, we define the Hamming distance (or, simply, distance) $d(\mathbf{a},\mathbf{b})$ between $\mathbf{a}$ and $\mathbf{b}$ as the number of coordinates in which they differ, i.e., $d(\mathbf{a},\mathbf{b}) = |\{i\in [n]:\ a_i\neq b_i\}|$.  Further, given a length-$n$ vector $\mathbf{a}$, let $a_i^j$ denote the vector $(a_k:\ i\leq k\leq j)$, for $i\geq 1$ and $j\leq n$. 
%Given a length $n$, we let $\mathbf{B}_n(i)$ denote the binary representation of $0\leq i\leq 2^n-1$. The subscript `$n$' will be dropped when evident from the context. 
%Further, for $\mathbf{z}\in \{0,1\}^n$, we define $w_\mathbf{z}(\mathbf{a})$ to be the number of ones in $\mathbf{a}$, in those positions $1\leq i\leq n$ where $z_i = 1$. 
For $r\in \{0,1\}$, we define the vector $r^m$ to be the length-$m$ vector all of whose symbols equal $r$. Further, given two binary vectors $\mathbf{a} = (a_1,\ldots,a_n)$ and $\mathbf{b} = (b_1,\ldots,b_n)$, their dot product $\mathbf{a}\cdot \mathbf{b}$ equals $\sum_{i=1}^n a_i b_i$, and we denote their concatenation by $\mathbf{a}\mathbf{b}$. 
%For an $m\times n$ matrix $M$, we use the notation $M[i]$ to denote its $i^{\text{th}}$ column, for $i\in [n]$, and $M(j)$ to denote its $j^{\text{th}}$ row, for $j\in [m]$. 
For a given real number $r\in \mathbb{R}$, we define $\left \lfloor r\right \rfloor$ and $\left \lceil r\right \rceil$ to be, respectively, the largest integer less than or equal to $r$, and the smallest integer larger than or equal to $r$. Further, for integers $p$, $r$, and $n$, with $n>0$ and $1\leq r\leq n$, we say that $p\equiv r\ (\text{mod }n)$, or that $r = \text{mod}(p,n)$, if $p = qn+r$, for some integer $q$.
For a set $P$ and $\mathbf{x}\in \{0,1\}^n$, we use the notation $$\mathds{1}_{P}(\mathbf{x}) = \begin{cases}1,\ \text{if $\mathbf{x}\in P$},\\0,\ \text{otherwise,}\end{cases}$$ and we write $\mathds{1}_P$ as the indicator function $\left(\mathds{1}_P(\mathbf{x}):\ \mathbf{x}\in \{0,1\}^n\right)$.
\subsection{Block Codes and Constrained Codes}
We recall the following definitions of block codes over $\mathbb{F}_2$ (see, for example, Chapters 1 and 2 of \cite{roth_coding_theory}).

\begin{definition}
	An $(n,M)$ block code $\mathcal{C}$ over $\mathbb{F}_2$ is a nonempty subset of $\mathbb{F}_2^n$, with $|\mathcal{C}| = M$. The rate of the block code $\mathcal{C}$ is given by
	\[
	\text{rate}(\mathcal{C}) := \frac{\log_2 M}{n}.
	\]
\end{definition}
\begin{definition}
	The minimum distance $d(\mathcal{C})$ of a block code $\mathcal{C}$ is the minimum distance between any two distinct codewords of $\mathcal{C}$, i.e., 
	\[
	d(\mathcal{C}) = \min_{\mathbf{c}_1,\mathbf{c}_2\in \mathcal{C}:\ \mathbf{c}_1\neq \mathbf{c}_2} d(\mathbf{c}_1,\mathbf{c}_2).
	\]
\end{definition}
An $(n,M)$ block code with minimum distance $d$ will be called an $(n,M,d)$ block code. 

In this work, we shall be concerned with binary words that lie in a certain set $\mathcal{A}\subseteq \{0,1\}^n$. We shall call such words as ``constrained words'' or ``constrained sequences'', and refer to a block code $\mathcal{C}$, all of whose codewords lie in $\mathcal{A}$, as a ``constrained code''. We refer the reader to \cite{Roth} for a detailed exposition on constrained sequences and coding in the presence of constraints. Note that we make no further assumption about the constrained system (such as it being finite-type, almost-finite-type, irreducible, etc.). For a given blocklength $n$, we use the notation $A(n,d;\mathcal{A})$ to denote the size of the largest constrained code, of minimum distance at least $d$, such that all of its codewords lie in $\mathcal{A}$. More formally,
\[
A(n,d;\mathcal{A}):= \max_{\substack{\mathcal{C}\subseteq \mathcal{A}:\ d(\mathcal{C})\geq d}} |\mathcal{C}|.
\]
For the case where $\mathcal{A} = \{0,1\}^n$, we write $A(n,d;\mathcal{A})$ as simply $A(n,d)$.
%%Consider now a set $S^{(n)}$ of length-$n$ binary words that satisfy the $(d,\infty)$-RLL constraint. We recall the following definition (see, for example, Chapter 3 of \cite{Roth}):
%%\begin{definition}
%%	The noiseless capacity $C_0^{(d)}$ of the $(d,\infty)$-RLL constraint is defined as
%%	\[
%%	C_0^{(d)}:= \lim_{n\to \infty} \frac{\log_2\left\lvert S_{(d,\infty)}^{(n)}\right \rvert}{n} = \inf_n \frac{\log_2\left\lvert S_{(d,\infty)}^{(n)}\right \rvert}{n},
%%	\]
%%	where the last equality follows from the subadditivity of the sequence $\left(\log_2\left\lvert S_{(d,\infty)}^{(n)}\right\rvert\right)_{n\geq 1}$. 
%\end{definition}
\subsection{Fourier Expansions of Boolean Functions}
\label{sec:fourierprelim}
Consider functions $f: \{0,1\}^n\to \mathbb{R}$, mapping $\mathbf{x} = (x_1,\ldots,x_n) \in \{0,1\}^n$ to $f(\mathbf{x})\in \mathbb{R}$. If the range of $f$ is $\{0,1\}$, then $f$ is called a Boolean function.  Now, given any function $f: \{0,1\}^n\to \mathbb{R}$ and a vector $\mathbf{s} = (s_1,\ldots,s_n)\in \{0,1\}^n$, we define the Fourier coefficient of $f$ at $\mathbf{s}$ as
\[
\widehat{f}(\mathbf{s}):= \frac{1}{2^n}\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x})\cdot (-1)^{\mathbf{x}\cdot \mathbf{s}}.
\]
The function $\widehat{f}$ is known as the Fourier transform of $f$. Note that the Fourier transform operation is linear, i.e., if $f = a\cdot g+b\cdot h$, where $a,b\in \mathbb{R}$, then $\widehat{f}=a\cdot \widehat{g}+b\cdot \widehat{h}$. Moreover, the functions $\left(\chi_{\mathbf{s}}: \mathbf{s}\in \{0,1\}^n\right)$, where $\chi_{\mathbf{s}}(\mathbf{x}):=(-1)^{\mathbf{x}\cdot \mathbf{s}}$, form a basis for the vector space $V$ of functions $f: \{0,1\}^n\to \mathbb{R}$. The function $\chi_{\mathbf{s}}$ is also referred to as the Fourier character at $\mathbf{s}\in \{0,1\}^n$.  If we define an inner product $\langle \cdot, \cdot \rangle$ over the vector space $V$, as follows:
\[
\langle f,g \rangle := \frac{1}{2^n}\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x}) g(\mathbf{x}),
\]
for functions $f,g \in V$, we also have that the basis functions $\left(\chi_{\mathbf{s}}: \mathbf{s}\in \{0,1\}^n\right)$ are orthonormal, in that
\[
\langle \chi_{\mathbf{s}},\chi_{\mathbf{s}^\prime} \rangle = 
\begin{cases}
	1,\ \text{if $\mathbf{s} = \mathbf{s}^\prime$},\\
	0,\ \text{otherwise.}
\end{cases}
\]
The above discussion leads us to the following well-known theorem:
\begin{theorem}[Theorem 1.1 in \cite{ryanodonnell}]
	Every function $f: \{0,1\}^n\to \mathbb{R}$ can be uniquely expressed as its Fourier expansion
	\[
	f(\mathbf{x}) = \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{f}(\mathbf{s})\cdot (-1)^{\mathbf{x}\cdot \mathbf{s}}.
	\]
\end{theorem}
We recall Plancherel's Theorem, without proof, below.
\begin{theorem}[Plancherel's Theorem]
	For any $f,g \in \{0,1\}^n\to \mathbb{R}$, we have that
	\[
	\langle f,g \rangle = \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{f}(\mathbf{s})\widehat{g}(\mathbf{s}).
	\]
\end{theorem}
We also recall the operation of convolution of two functions $f,g: \{0,1\}^n\to \mathbb{R}$, defined as
\[
f\star g(\mathbf{x}) = \frac{1}{2^n}\sum_{\mathbf{z}\in \{0,1\}^n} f(\mathbf{z})\cdot g(\mathbf{x}+\mathbf{z}),
\]
where the `$+$' operation in $\mathbf{x}+\mathbf{z}$ above is over vectors in $\mathbb{F}_2^n$.

It is well-known (see \cite{ryanodonnell}) that the Fourier transform
\[
\widehat{f\star g}(\mathbf{s}) = \widehat{f}(\mathbf{s})\cdot \widehat{g}(\mathbf{s}),
\]
%We also recollect Plancherel's Theorem from Fourier analysis, below, without proof.
%\begin{theorem}[Plancherel's Theorem]
%	For any $f,g \in \{0,1\}^n\to \mathbb{R}$, we have that
%	\[
%	\langle f,g \rangle = \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{f}(\mathbf{s})\widehat{g}(\mathbf{s}).
%	\]
%\end{theorem}
for any $\mathbf{s}\in \{0,1\}^n$. For more details on the Fourier analysis of Boolean functions, we refer the reader to \cite{ryanodonnell}. 



==> appa.tex <==
\section{On the Weight Distribution of Constrained Sequences in $\mathbb{F}_2^n$}
\label{sec:appa}
Suppose that we are interested in computing the weight distribution of words in $\{0,1\}^n$ that lie in a (constrained) set $\mathcal{A}\subseteq \{0,1\}^n$. Let $a_{i,\mathcal{A}}$ denote the number of constrained words of weight $i\in [0:n]$ and recall the definition of the $i^\text{th}$-Krawtchouk polynomial $K_i^{(n)}$, for a given blocklength $n$, where $K_i^{(n)}(z) = \sum_{\ell=0}^{i} (-1)^\ell {z\choose \ell} {n-z\choose i-\ell}$, and the notation $W_i=\{\mathbf{x}\in \{0,1\}^n: w(\mathbf{x}) = i\}$. The following theorem then holds true:

\begin{theorem}
	\label{thm:wtcount}
	The weight distribution of sequences that lie in a set $\mathcal{A}\subseteq \{0,1\}^n$ obeys
	\[
	a_{i,\mathcal{A}} = \sum_{j=0}^n K_i^{(n)}(j)\cdot \sum_{\mathbf{s}:\ w(\mathbf{s}) = j} \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s}),\quad i\in [0:n].
	\]
\end{theorem}
\begin{proof}
	The proof is again a simple application of Plancherel's Theorem. Observe that
	\begin{align}
		a_{i,\mathcal{A}} &\stackrel{}{=} \sum_{\mathbf{x}\in \mathcal{A}} \mathds{1}_{W_i}(\mathbf{x}) \notag\\
		&= \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_{W_i}(\mathbf{x})\cdot \mathds{1}_{\mathcal{A}}(\mathbf{x})  \notag \\
		&= 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\mathds{1}_{W_i}}(\mathbf{s})\cdot \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s})  \label{eq:inter2}.
	\end{align}
	%where in (a) we use the notation $W_i:=\{\mathbf{x}\in \{0,1\}^n: w(\mathbf{x}) = i\}$. 
	We now recall the well-known proof of the fact that  $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}) = K_i(w(\mathbf{s}))$ (see Chapter 5 in \cite{mws} for more details on Krawtchouk polynomials). Note that
	\begin{align*}
		2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s})  = \sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i} (-1)^{\mathbf{x}\cdot \mathbf{s}}.
	\end{align*}
	Now, the summation on the right side depends only on the weight $w(\mathbf{s})$, i.e., for any permutation of coordinates $\pi: \{0,1\}^n\to \{0,1\}^n$, it holds that
	\begin{align*}
		\sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i}	(-1)^{\mathbf{x}\cdot \pi(\mathbf{s})} &= \sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i}  (-1)^{\pi(\mathbf{x})\cdot \pi(\mathbf{s})}\\
		&= \sum_{\mathbf{x}\in \{0,1\}^n:\ w(\mathbf{x}) = i} (-1)^{\mathbf{x}\cdot \mathbf{s}}.
	\end{align*}
	In other words, we have that $\widehat{\mathds{1}_{W_i}}(\mathbf{s}) = \widehat{\mathds{1}_{W_i}}(\pi(\mathbf{s}))$. Hence, for $\mathbf{s}$ such that $w(\mathbf{s}) = j$, it suffices that we calculate $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}^\star)$, where $\mathbf{s}^\star = (s_1^\star,\ldots,s_n^\star)$ is such that $s_1^\star = \ldots = s_j^\star = 1$ and $s_{j+1}^\star=\ldots=s_n^\star = 0$. By a direct computation, it can be checked that $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}^\star) = \sum_{\ell=0}^{i} (-1)^\ell {j\choose \ell} {n-j\choose i-\ell} = 2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s})$. Plugging this back into \eqref{eq:inter2} and simplifying, we obtain the expression in the theorem.
\end{proof}
%As before, Theorem \ref{thm:wtcount} implies that if the Fourier coefficients $\widehat{\mathds{1}_\mathcal{A}}(\mathbf{s})$ (or, the sum of Fourier coefficients at a fixed weight $\sum_{\mathbf{s}:\ w(\mathbf{s}) = j} \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s})$) were available to us, we can easily compute the number of constrained words of a given weight.

==> appb.tex <==
\section{Weight Distribution of Constrained Codewords in Linear Codes}
\label{sec:appb}
In this section, we briefly describe another useful computation that is facilitated by knowledge of the Fourier coefficients of the indicator function that a word belongs to a set of constrained sequences. Before we do so, we recall another property of Fourier transforms:
\begin{theorem}
	\label{thm:conv}
	Given functions $f,g:\{0,1\}^n\to \mathbb{R}$, the Fourier transform of $f\cdot g$ is the function $\widehat{f}\ostar \widehat{g}$, where
	\[
	(\widehat{f}\ostar \widehat{g}) (\mathbf{s}) := \sum_{\mathbf{z}\in \{0,1\}^n}\widehat{f}(\mathbf{z})\widehat{g}(\mathbf{z}+\mathbf{s}) = 2^n\cdot (\widehat{f}\star \widehat{g})(\mathbf{s}),\quad \mathbf{s}\in \{0,1\}^n.
	\]
\end{theorem}

The calculation we wish to perform puts together the theses of Theorems III.1 of the paper and I.1 of the supplement. In particular, we ask for the number of codewords of a linear code $\mathcal{C}$, which lie in a fixed set $\mathcal{A}$ and are of a given weight. We thus obtain Theorem \ref{thm:linwtcount}. For a given $\mathbf{v}\in \{0,1\}^n$, we use the notation $\mathbf{v}+\mathcal{C}$ to denote the coset of $\mathcal{C}$ to which $\mathbf{v}$ belongs. We let $a_{i,\mathcal{A}}(\mathcal{C})$ denote the number of constrained codewords of weight $i\in [0:n]$, which lie in the set $\mathcal{A}$ and in a linear code $\mathcal{C}$.
\begin{theorem}
	\label{thm:linwtcount}
	Given a linear code $\mathcal{C}$ of blocklength $n$, we have that
	\[
	a_{i,\mathcal{A}}(\mathcal{C}) = \frac{\left\lvert \mathcal{C}\right\rvert}{2^n} \sum_{j=0}^n K_i^{(n)}(j) \sum_{\mathbf{s}:\ w(\mathbf{s}) = j} \sum_{\mathbf{z}\in \mathbf{s}+\mathcal{C}^\perp} \widehat{\mathds{1}_{\mathcal{A}}} (\mathbf{z}).
	\]
\end{theorem}
\begin{proof}
	We observe that
	\begin{align*}
		a_{i,\mathcal{A}}(\mathcal{C}) &= \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_{W_i}(\mathbf{x})\cdot \mathds{1}_{\mathcal{A}}(\mathbf{x})\cdot \mathds{1}_{\mathcal{C}}(\mathbf{x})\\
		&{=} 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\mathds{1}_{W_i}}(\mathbf{s})\cdot \widehat{\mathds{1}_{\mathcal{A}}\cdot \mathds{1}_{\mathcal{C}}}(\mathbf{s}),
	\end{align*}
	where the last equality above uses Plancherel's Theorem (see Theorem II.1 of the paper). Further, by employing Theorem \ref{thm:conv} to expand the last equality, we get that
	\begin{align*}
		a_{i,\mathcal{A}}(\mathcal{C})&= 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\mathds{1}_{W_i}}(\mathbf{s})\cdot \left(\widehat{\mathds{1}_{\mathcal{A}}}\ostar \widehat{\mathds{1}_{\mathcal{C}}}\right)(\mathbf{s})\\
		&\stackrel{(a)}{=} \frac{\left\lvert \mathcal{C}\right\rvert}{2^n}\cdot \sum_{\mathbf{s}\in \{0,1\}^n} K_i^{(n)}(w(\mathbf{s}))\sum_{\mathbf{z}\in \{0,1\}^n} \widehat{\mathds{1}_{\mathcal{C}^\perp}}(\mathbf{z})\cdot \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s}+\mathbf{z})\\
		&= \frac{\left\lvert \mathcal{C}\right\rvert}{2^n} \cdot  \sum_{j=0}^n K_i^{(n)}(j) \sum_{\mathbf{s}:\ w(\mathbf{s}) = j}\ \sum_{\mathbf{z}\in \mathbf{s}+\mathcal{C}^\perp} \widehat{\mathds{1}_{\mathcal{A}}} (\mathbf{z}),
	\end{align*}
	where equality (a) above uses the fact that $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}) = K_i^{(n)}(w(\mathbf{s}))$ and that $\widehat{\mathds{1}_{\mathcal{C}}}(\mathbf{s}) = \frac{\left\lvert \mathcal{C}\right\rvert}{2^n}\cdot \mathds{1}_{\mathcal{C}^\perp}(\mathbf{s})$ (see the proofs of Theorems III.1 in the paper and I.1 in the supplement).% \ref{thm:wtcount} and \ref{thm:lincount}).
\end{proof}

Theorem \ref{thm:linwtcount} could prove useful in the following context: consider the transmission of codewords of a linear code $\mathcal{C}$ over an input-constrained binary-input memoryless symmetric (BMS) channel, which admits only binary constrained sequences that lie in the set $\mathcal{A}$ as inputs. Suppose that the decoder being used is the maximum a-posteriori (MAP) (equivalently, the maximum likelihood (ML)) decoder of the linear code $\mathcal{C}$. By calculating the weight distribution of constrained codewords in a linear code $\mathcal{C}$ as above, it is possible to obtain an upper bound on the block error probability (via a union bounding argument), when the MAP decoder is used (see Chapter 1 of \cite{mct}).

==> appd.tex <==
\section{An Upper Bound on $\text{val}(\mathsf{Del}(n,d;\mathcal{A}))$}
In this section, similar to the approach in \cite{linial2} we derive an upper bound on the optimal value val$(\mathsf{Del}(n,d;\mathcal{A}))$ of our LP, in the following lemma that is essentially a formulation of the dual LP. We believe that the lemma will be useful in the derivation of asymptotic (as the blocklength goes to infinity) upper bounds on the rate-distance tradeoff for constrained codes. We abbreviate $	\text{val}(\mathsf{Del}(n,d))$ as $v$ and $\text{val}(\mathsf{Del}(n,d;\mathcal{A}))$ as $v_\mathcal{A}$.

\begin{lemma}
	\label{lem:dual}
	Let $\beta: \{0,1\}^n \to \mathbb{R}$ be a function that satisfies
	\begin{enumerate}
		\item $\widehat{\beta}(\mathbf{s})\geq 0$, for all $\mathbf{s}\in \{0,1\}^n$,
		\item $\beta(\mathbf{s})\leq 0$, if $w(\mathbf{s})\geq d$, and
		\item $\sum_{\mathbf{x}}\beta(\mathbf{x}) = 2^n$.
	\end{enumerate}
Then, it holds that
	$
	v_\mathcal{A}\leq \beta(0^n)\cdot \min\{v,|\mathcal{A}|\}.
	$
\end{lemma}
\begin{proof}
	Consider any function $\beta: \{0,1\}^n\to \mathbb{R}$ that satisfies the conditions in the statement of the lemma. Now, observe that for any feasible solution $f$ of $\mathsf{Del}(n,d;\mathcal{A})$, we have that
	\begin{align*}
		\widehat{\beta}(0^n)\cdot \widehat{f}(0^n)&\stackrel{(a)}{\leq} \sum_{\mathbf{x}\in \{0,1\}^n}\widehat{\beta}(\mathbf{x})\cdot \widehat{f}(\mathbf{x})\\
		&\stackrel{(b)}{=} \frac{1}{2^n}\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \beta(\mathbf{s})\cdot {f(\mathbf{s})}\\
		&\stackrel{(c)}{=} \frac{1}{2^n}\cdot \sum_{\substack{\mathbf{s}:\ \mathbf{s}\ =\ 0^n\text{ or }\\w(\mathbf{s})\geq d}} \beta(\mathbf{s})\cdot f(\mathbf{s})\\
		&\stackrel{(d)}{\leq} 2^{-n}\cdot\beta(0^n)\cdot \min\{v,|\mathcal{A}|\},
	\end{align*}
	where (a) holds since $\lambda, \widehat{f}\geq 0$ and (b) holds by an application of Plancherel's Theorem. Next, (c) is true since $f$ satisfies (D3) and (d) holds since $f$ satisfies (D4) and (D5), and from item 2) in the statement of the lemma, and also since $2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(0^n) = |\mathcal{A}|$.
	
	Moreover, we have that val$(f) = \sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x}) = 2^n\cdot \widehat{f}(0^n)$, and that $\widehat{\beta}(0^n) = \frac{1}{2^n} \sum_{\mathbf{x}\in \{0,1\}^n} \beta(\mathbf{x}) = 1$, by the definition of the Fourier transform. Putting everything together, we obtain that for any feasible $f$ of $\mathsf{Del}(n,d;\mathcal{A})$, it holds that
	$
	\text{val}(f)\leq \beta(0^n)\cdot \min\{v,|\mathcal{A}|\}.
	$
	The statement of the lemma then follows.
\end{proof}
%Using results from \cite{linial2}, it is now possible to prove Proposition III.3.
%\begin{proof}[Proof of Proposition III.3]
%	From the discussion in Section 2.3 of \cite{linial2}, it follows that there exists a function $\beta: \{0,1\}^n\to \mathbb{R}$ that satisfies items 1)--3) of Lemma \ref{lem:dual}, such that $\limsup_{n\to \infty} \frac{\log_2 \beta(0^n)}{n}\leq h_b(1/2+\sqrt{\delta(1-\delta)})$. From Theorem III.3 and Lemma \ref{lem:dual}, we then have that
%	\[
%	\limsup_{n\to \infty} \frac{1}{n}\cdot{\log_2A(n,\left \lfloor \delta n\right \rfloor;\mathcal{A}_n)} \leq \frac{1}{2}\cdot \limsup_{n\to \infty} \frac{ \log_2 v_{\mathcal{A}_n}}{n}\leq \min\left\{C_0,\frac{1}{2}\cdot \left(C_0+h_b(1/2+\sqrt{\delta(1-\delta)})\right)\right\},
%	\]
%	where $C_0 = \limsup_{n\to \infty} \frac{1}{n}\cdot \log_2|\mathcal{A}_n|$ is the noiseless capacity
%\end{proof}

==> appf.tex <==
\section{Proof of Lemma IV.5}
\begin{proof}
	To prove the first recurrence relation, we write
	\begin{align}
	\widehat{\mathds{1}_{S^{d}}}^{(n)}(\mathbf{s}) &= \frac{1}{2^n}\cdot \sum_{\mathbf{x}\in S^d} (-1)^{\mathbf{x}\cdot \mathbf{s}} \notag\\
	&= 2^{-n}\cdot\left(\#\{x^n\in S^d:\ w_\mathbf{s}(x^n)\text{ is even}\} - \#\{x^n\in S^d:\ w_\mathbf{s}(x^n)\text{ is odd}\}\right). \label{eq:inter8}
	\end{align}
Now, observe that
\begin{align}
	\#\{x^n\in S^d:\ w_\mathbf{s}(x^n)\text{ is even}\} &= \#\{x^n\in S^d:\ w_\mathbf{s}(x^n)\text{ is even and $x_1 = 0$}\}\ +\notag\\&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \#\{x^n\in S^d:\ w_\mathbf{s}(x^n)\text{ is even and $x_1 = 1$}\} \notag\\
	&\stackrel{(a)}{=} \#\{x_2^n\in S^d:\ w_{s_2^n}(x_2^n)\text{ is even}\}\ + \notag\\&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
	\#\{x^n\in S^d:\ w_\mathbf{s}(x^n)\text{ is even and $x_1^{(d+1)} = 10^d$}\} \notag\\
	&=  \#\{x_2^n\in S^d:\ w_{s_2^n}(x_2^n)\text{ is even}\} + \#\{x_{d+2}^n\in S^d:\ w_{s_{d+2}^n}(x^n)\text{ is even}\}, \label{eq:inter9}
\end{align}
where (a) holds because $s_1 = 0$ and from the fact that the $(d,\infty)$-RLL constraint requires that $x_2^{d+1} = 0^d$, if $x_1 = 1$. Similarly, we obtain that
\begin{align}
	\#\{x^n\in S^d:\ w_\mathbf{s}(x^n)\text{ is odd}\}
	&=  \#\{x_2^n\in S^d:\ w_{s_2^n}(x_2^n)\text{ is odd}\} + \#\{x_{d+2}^n\in S^d:\ w_{s_{d+2}^n}(x^n)\text{ is odd}\}. \label{eq:inter10}
\end{align}
Now, observe that
\begin{equation}
	\label{eq:inter14}
\widehat{\mathds{1}_{S^{d}}}^{(n-1)}(s_2^n) = 2^{-(n-1)}\cdot\left(\#\{x_2^n\in S^d:\ w_{s_2^n}(x_2^n)\text{ is even}\} - \#\{x_2^n\in S^d:\ w_{s_2^n}(x_2^n)\text{ is odd}\}\right)
\end{equation}
and that
\begin{align}
\widehat{\mathds{1}_{S^{d}}}^{(n-d-1)}(s_{d+2}^n) = 2^{-(n-d-1)}\cdot\Big(\#\{x_{d+2}^n\in S^d:\ w_{s_{d+2}^n}(x_{d+2}^n)&\text{ is even}\} - \notag\\& \#\{x_{d+2}^n\in S^d:\ w_{s_{d+2}^n}(x_{d+2}^n)\text{ is odd}\}\Big).	\label{eq:inter15}
\end{align}
Substituting \eqref{eq:inter9} and \eqref{eq:inter10} in \eqref{eq:inter8} and using \eqref{eq:inter14} and \eqref{eq:inter15}, we get the first recurrence relation. The second recurrence relation is also proved by similar arguments.
\end{proof}

==> conclusion.tex <==
\label{sec:conclusion}

In this work, we demonstrated an extension of Delsarte's linear program (LP), whose optimal value is an upper bound on the size of a constrained code of length $n$ and minimum distance at least $d$, for an arbitrary constraint represented by a set $\mathcal{A}\subseteq \{0,1\}^n$ of constrained sequences. For select constraints, we showed that it is in fact possible to reduce the number of variables and LP constraints, by a symmetrization procedure that makes use of a certain subgroup of coordinate permutations that leaves the indicator function of the constraint invariant. We then applied our LP to different constraints, and observed that the optimal numerical values returned by our LP are better than those provided by the generalized sphere packing bounds of Fazeli, Vardy, and Yaakobi (2015).

An interesting direction for future work would be to use the dual LP formulation in this paper to derive asymptotic (in the limit as the blocklength goes to infinity) upper bounds on the rate-distance tradeoff for constrained codes. This will help us understand if the Gilbert-Varshamov lower bounds of Kolesnik and Krachkovsky (1991) and Marcus and Roth (1992) are tight for any constrained system.

==> even.tex <==
\label{sec:even}
We now move on to the so-called even constraint, which, analogous to the odd constraint discussed in Section \ref{sec:odd}, admits only binary sequences that have an even number of $0$s between successive $1$s. The even constraint is often used in conjunction with $(d,k)$-RLL constraints, in magneto-optical recording systems (see \cite{even1}). The overall constraint is written as the $(d,k,2)$-RLL constraint. A prototype for such a system was built by IBM \cite{odd1,odd2,even2}. In this paper, we impose the additional constraint that the lengths of the first and last (leading and trailing) runs of $0$s also be even. We let $S_{\text{e}^\star}^{(n)}$ (or, $S_{\text{e}^\star}$) denote the set of such binary sequences of length $n$, with the convention that the all-zeros sequence $0^n \in S_{\text{e}^\star}^{(n)}$, for all $n\geq 1$.

As before, for $n\geq 1$, and for $\mathbf{s}\in \{0,1\}^n$, let $\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n)}(\mathbf{s})$ denote the Fourier coefficient at $\mathbf{s}$, when the blocklength is $n$. The following sets of recurrence relations then hold true:
\begin{lemma}
	\label{lem:fcoeffeven}
	For $n\geq 3$ being even and for $\mathbf{s} = (s_1,\ldots,s_n)\in \{0,1\}^n$, it holds that when $s_1 = 0$, 
	\[
	\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n)}(\mathbf{s}) = 2^{-1}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-1)}(s_2^n)+2^{-2}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-2)}(s_3^n)-\frac{1}{2^n},
	\]
	and when $s_1 = 1$, 
	\[
	\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n)}(\mathbf{s}) = 2^{-2}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-2)}(s_3^n)-2^{-1}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-1)}(s_2^n)+\frac{1}{2^n}.
	\]
	Further, for $n\geq 3$ being odd, it holds that when $s_1 = 0$, 
	\[
	\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n)}(\mathbf{s}) = 2^{-1}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-1)}(s_2^n)+2^{-2}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-2)}(s_3^n),
	\]
	and when $s_1 = 1$, 
	\[
	\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n)}(\mathbf{s}) = 2^{-2}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-2)}(s_3^n)-2^{-1}\cdot\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-1)}(s_2^n).
	\]
\end{lemma}
\begin{proof}
	We shall prove only the first of the four recurrence relations above. The proofs of the remaining recurrences are similar and are hence omitted. To prove the first recurrence relation in the case when $n$ is even, we write as before
		\begin{align}
		\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n)}(\mathbf{s}) &= \frac{1}{2^n}\cdot \sum_{\mathbf{x}\in S_{\text{e}^\star}} (-1)^{\mathbf{x}\cdot \mathbf{s}} \notag\\
		&= 2^{-n}\cdot\left(\#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is even}\} - \#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is odd}\}\right). \label{eq:inter11}
	\end{align}
	Now, note that
	\begin{align}
		\#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is even}\} &= \#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is even and $x_1 = 0$}\} + \#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is even and $x_1 = 1$}\} \notag\\
		&\stackrel{(a)}{=} \#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is even and $x_1 = x_2= 0$}\} + 
		\#\{x_2^n\in S_{\text{e}^\star}:\ w_{s_2^n}(x_2^n)\text{ is even}\} -1 \notag\\
		&=  \#\{x_3^n\in S_{\text{e}^\star}:\ w_{s_3^n}(x_3^n)\text{ is even}\} +\#\{x_2^n\in S_{\text{e}^\star}:\ w_{s_2^n}(x_2^n)\text{ is even}\} -1, \label{eq:inter12}
	\end{align}
where in (a) above, we have that $x_2 = 0$ if $x_1 = 0$, owing to the constraint that the leading run of $0$s must be of even length, and that $\#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is even and $x_1 = 1$}\} = \#\{x_2^n\in S_{\text{e}^\star}:\ w_{s_2^n}(x_2^n)\text{ is even}\}-1$, since if $x_1 = 1$ and $n$ is even, it cannot be that $x_2^n = 0^{n-1}$, since then the trailing run of $0$s will be of odd length.

Similarly, we have that
\begin{equation}
	\label{eq:inter13}
\#\{x^n\in S_{\text{e}^\star}:\ w_\mathbf{s}(x^n)\text{ is odd}\} =  \#\{x_3^n\in S_d:\ w_{s_3^n}(x_3^n)\text{ is odd}\} +\#\{x_2^n\in S_{\text{e}^\star}:\ w_{s_2^n}(x_2^n)\text{ is odd}\}.
\end{equation}
Note that since in the second expression on the right-hand side above, we require that $w_{s_2^n}(x_2^n)$ be odd, the all-zeros sequence $x_2^n = 0^{n-1}$ is already ruled out, and we thus do not need to subtract $1$ as in \eqref{eq:inter12}. 

Furthermore, observe that
\begin{equation}
	\label{eq:inter16}
	\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-1)}(s_2^n) = 2^{-(n-1)}\cdot\left(\#\{x_2^n\in S_{\text{e}^\star}:\ w_{s_2^n}(x_2^n)\text{ is even}\} - \#\{x_2^n\in S_{\text{e}^\star}:\ w_{s_2^n}(x_2^n)\text{ is odd}\}\right)
\end{equation}
and that
\begin{equation}
	\label{eq:inter17}
	\widehat{\mathds{1}_{S_{\text{e}^\star}}}^{(n-2)}(s_{3}^n) = 2^{-(n-2)}\cdot\left(\#\{x_{3}^n\in S_{\text{e}^\star}:\ w_{s_{3}^n}(x_{3}^n)\text{ is even}\} - \#\{x_{3}^n\in S_{\text{e}^\star}:\ w_{s_{3}^n}(x_{3}^n)\text{ is odd}\}\right).
\end{equation}
Plugging \eqref{eq:inter12} and \eqref{eq:inter13} into \eqref{eq:inter11} and using \eqref{eq:inter16} and \eqref{eq:inter17}, we obtain the first recurrence relation.
\end{proof}

As in the previous subsection, we have that the computation of the Fourier coefficients for a given blocklength $n$, by iteratively applying Lemma \ref{lem:fcoeffeven} offers significant computation time savings as compared to using the FWHT algorithm. Indeed, here too, the time required for computing the Fourier coefficients at blocklength $n$ is at most $2^{n+1}$, assuming that the additions and multiplications in Lemma \ref{lem:fcoeffeven} take unit time, while the time required for a run of the FWHT algorithm is of the order of $n\cdot 2^n$. Once again, it also holds that the storage cost of saving the Fourier coefficients for blocklengths $n\gtrapprox 20$ is quite expensive, regardless of whether the computation of Fourier coefficients is performed using the FWHT algorithm or using our recursive procedure.

Furthermore, we use the Fourier coefficients that are numerically computed using Lemma \ref{lem:fcoeffeven}, to compute the number of codewords in select codes, which lie in $S_{\text{e}^\star}$, with the aid of Theorem \ref{thm:lincount}. The values are documented in Table \ref{tab:rmeven}. We also use Theorem \ref{thm:wtcount} to calculate the weight distributions of words that lie in $S_{\text{e}^\star}$, for large blocklengths $n$. The weight distribution of constrained words when $n=17$ is shown in Table \ref{tab:wteven}.
\begin{table}[t!]
	\centering
	\begin{tabular}{||c || c||} 
		\hline
		$\mathcal{C}$ & $N(\mathcal{C};S_{\text{e}^\star})$\\ [0.5ex] 
		\hline\hline
		RM$(4,2)$ & $198$\\ 
		\hline
		RM$(4,3)$ & $1597$\\ 
		\hline
		Ham$_3$ & $6$\\
		\hline
		Ham$_4$ & $116$\\
		\hline
	\end{tabular}
	\caption{Table of values of $N(\mathcal{C};S_{\text{e}^\star})$, for select codes $\mathcal{C}$}
	\label{tab:rmeven}
\end{table}

\begin{table}[t!]
	\centering
	\begin{tabular}{||c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c ||} 
		\hline
		Weight $i$ & $0$& $1$& $2$& $3$& $4$& $5$& $6$ & $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$\\ [0.5ex] 
		\hline\hline
		$a_{i,S_{\text{e}^\star}}$ & $1$& $9$& $0$& $120$& $0$& $462$& $0$ & $792$ &$0$ &$715$ &$0$ &$364$ &$0$ &$105$ &$0$ &$16$ &$0$ &$1$\\ 
		\hline
	\end{tabular}
	\caption{Weight distribution $\left(a_{i,S_{\text{e}^\star}}:\ 0\leq i\leq n\right)$, when $n=17$}
	\label{tab:wteven}
\end{table}

==> introduction-fourier.tex <==
In the construction of binary linear codes, a code designer may sometimes want the codewords to satisfy additional properties. For example, if the codewords were intended to be written onto a magnetic disk, then the code designer may wish to avoid certain codewords that are more prone to error than others. {C}{onstrained} coding is a method that helps alleviate error-prone sequences in data recording and communication systems, by allowing the encoding of arbitrary user data sequences into only those sequences that respect the constraint (see, for example, \cite{Roth} or \cite{Immink}). Our interest in this paper is in subcodes of linear codes that respect a fixed constraint. 

One motivation for considering constrained subcodes of binary linear codes is the following: the data recording or communication medium can be thought of as a noisy channel that introduces errors stochastically. If the channel is memoryless and symmetric, besides, there are well-known binary linear codes that achieve the capacity or whose rates are very close to the capacity of the channel (see \cite{polar, Reeves,ru1}). In particular, this means that constrained subcodes of such linear codes also enjoy vanishing error probabilities over such binary-input memoryless symmetric (BMS) channels, in the limit as the blocklength goes to infinity. This observation can be useful for the construction of constrained coding schemes of good rates over input-constrained BMS channels, without feedback \cite{arnk22titarxiv}. We mention here that the problem of constructing codes over input-constrained memoryless channels, which form a special class of finite-state channels (FSCs), is still wide open.

In this paper, hence, we shall concern ourselves with the computation of the sizes of (arbitrarily) constrained subcodes of general linear codes. Our approach makes use of a simple identity from the Fourier analysis of Boolean functions, namely, Plancherel's Theorem, which transforms our counting problem to one in the space of the dual code. An immediate advantage of this approach is that the dimension of the vector space over which we count, which is the minimum of the dimensions of the linear code and its dual, is always bounded above by half the blocklength of the code. We also show, using specific examples of constraints, that our approach can yield not just the values of the sizes of constrained subcodes of specific linear codes, but also interesting insights into the construction of linear codes with a presribed number of constrained codewords. An artefact of our method is the Fourier transform of the indicator function that a word is constrained---an object that we believe is of independent interest. We show that in the cases of certain constraints, this Fourier transform is explicitly computable, and in some others, is efficiently calculable via a recursive procedure. We also apply our Fourier-analytic approach to the problem of computing the weight distributions of constrained words in the ambient space $\mathbb{F}_2^n$, where $n$ is the blocklength, and within the linear code $\mathcal{C}$ of interest.

The remainder of the paper is organized as follows: Section \ref{sec:preliminaries} establishes notation,  refreshes some background on linear codes and elementary Fourier analysis on the hypercube, and introduces the main theorems. Section \ref{sec:appl1} takes up examples of constraints wherein the Fourier transform of the indicator function of the constraint is explicitly computable, and discusses the ramifications of the theorems in Section \ref{sec:preliminaries}. Section \ref{sec:appl2} contains examples of constraints wherein the aforementioned Fourier transform is efficiently computable, numerically, and provides applications of the theorems in Section \ref{sec:preliminaries} to such constraints. Next, Section \ref{sec:wtdistlin} briefly outlines a method to compute the weight distributions of constrained codewords in a linear code. The paper is then concluded in Section \ref{sec:conclusion}, with some directions for future work.



==> introduction.tex <==
\IEEEPARstart{C}{onstrained} coding is a method that helps alleviate error-prone sequences in data recording and communication systems, by allowing the encoding of arbitrary user data sequences into only those sequences that respect the constraint (see, for example, \cite{Roth} or \cite{Immink}). In this paper, we are interested in determining the resilience of binary constrained codes to bit-flip errors or erasures. Since the error/erasure-correcting capability of codes is determined by their minimum Hamming distance, with a large minimum distance giving rise to better error/erasure correction, we shall try to obtain bounds on the largest sizes of constrained codes with a prescribed minimum distance.

There is extensive literature on the construction of and bounds for constrained codes with a certain minimum distance, and we refer the reader to Chapter 9 of \cite{Roth} for references. In particular, \cite{Ferreira} provided a simple lower bound on the sizes of runlength-limited (RLL) constrained codes with a given minimum Hamming distance, by a coset-averaging argument for linear codes. These bounds were then improved upon by Kolesnik and Krachkovsky \cite{kolesnik} and Marcus and Roth \cite{marcusroth}, via the solutions to certain constrained optimization problems. Less was known, in the case of upper bounds on constrained codes with a given minimum distance, until the works of Cullina and Kiyavash \cite{cullina} (see also \cite{kulkarni}) and Fazeli, Vardy, and Yaakobi \cite{fazeli}, which provided a generalization of the well-known sphere packing bound for codes, to the setting of constrained codes\footnote{While these papers were focussed on obtaining bounds on the sizes of codes for combinatorial error models, their techniques can be easily applied to determining upper bounds on the sizes of constrained codes with a given minimum distance as well.}. The approach in \cite{cullina} and \cite{fazeli} was based on finding the size of the largest matching, or equivalently, the size of the smallest transversal, in a suitably defined hypergraph. 

In this paper, we provide yet another approach to deriving good upper bounds on the sizes of constrained codes with a given minimum Hamming distance, by modifying Delsarte's well-known linear program (LP) \cite{delsarte} to the setting of constrained systems. While on a first pass, we propose an LP whose number of variables is exponential in the blocklength of the code, we show that for certain constraints, it is possible to ``symmetrize'' this LP to derive an equivalent LP with much smaller numbers of variables and constraints, which are sometimes only polynomial functions of the blocklength. We use our LPs to numerically calculate upper bounds on the sizes of the largest constrained codes with a prescribed minimum distance, for different constraints, and show that the values we obtain by our approach beats those obtained via the generalized sphere packing bounds. We believe that further study of our LP with the aid of modern Fourier-analytic techniques (see \cite{sam1,sam2}) could provide insight into asymptotic upper bounds on the rate-distance tradeoff for constrained codes.

The remainder of the paper is organized as follows: Section \ref{sec:preliminaries} puts down notation and refreshes some background on binary codes and elementary Fourier analysis on the hypercube. Section \ref{sec:lp} introduces our LP for constrained systems and provides some numerical examples. Section \ref{sec:sym} then defines a symmetrized version of our LP and specializes it to various constraints, while also providing numerical values of upper bounds for these constraints. The paper is then concluded in Section \ref{sec:conclusion} with some directions for future work.

==> lp.tex <==
\label{sec:lp}
In this section, we present a linear program (LP) to upper bound $A(n,d;\mathcal{A})$, for any $\mathcal{A}\subseteq \{0,1\}^n$. This LP is based on Delsarte's linear programming approach \cite{delsarte} to bounding from above the value of $A(n,d)$, for $n\geq 1$ and $1\leq d\leq n$. We first recall Delsarte's LP\footnote{The version of Delsarte's LP that is most often used in papers in coding theory, such as in \cite{mrrw}, is obtained after symmetrizing $\mathsf{Del}(n,d)$. In particular, the common version of Delsarte's LP is $\mathsf{Del}_{/S_n}(n,d)$ (see the remark following Theorem \ref{thm:equiv}), where $S_n$ is the symmetry group on $n$ elements.}, which we call $\mathsf{Del}(n,d)$. Given an LP $\mathsf{L}$, we denote by val$(\mathsf{L})$ its optimal value, and for any feasible solution $f$ of $\mathsf{L}$, we denote the value of the objective function of $\mathsf{L}$ evaluated at $f$ as val$_\mathsf{L}(f)$. The subscript will be omitted when the LP being referred to is clear from the context. We remark here that the LPs in this paper can return  non-integral optimal values, and that integer upper bounds on the sizes of codes can be obtained by suitable rounding of real numbers.
\begin{center}
	%	\begin{mybox}[colback=white, width = 0.75\linewidth]{$1,2$}
	%		This is my box.
	%	\end{mybox}
	\begin{tcolorbox}[title={\center $\mathsf{Del}(n,d)$}, title filled = false, width = 0.55\linewidth]
		\begin{align}
			&\underset{f:\ \{0,1\}^n\to \mathbb{R}}{\text{maximize}}\quad \sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x}) \tag{Obj}\\
			&\text{subject to:} \notag\\
			&\ \ f(\mathbf{x})\geq 0,\ \forall\ \mathbf{x}\in \{0,1\}^n, \tag{C1}\\
			&\ \ \widehat{f}(\mathbf{s})\geq 0,\ \forall\ \mathbf{s}\in \{0,1\}^n, \tag{C2}\\
			&\ \ f(\mathbf{x}) = 0,\ \text{if $1\leq w(\mathbf{x})\leq d-1$}, \tag{C3}\\
			&\ \ f(0^n) = 1. \tag{C4}
		\end{align}
	\end{tcolorbox}
\end{center}
Now, for any block code $\mathcal{C}$ of blocklength $n$ and minimum distance at least $d$, let $\mathds{1}_\mathcal{C}$ denote its indicator function. 
%If $\mathcal{C}$ does not contain the all-zeros word $0^n$, we translate the codewords of $\mathcal{C}$ so that it does contain the all-zeros word. Note that this translation operation preserves the distances between codewords, and hence the minimum distance of $\mathcal{C}$. 
Let us define\footnote{Note that when $\mathcal{C}$ is a linear code (or a subspace of $\mathbb{F}_2^n$), for all $\mathbf{x},\mathbf{z}\in \{0,1\}^n$, we have that $\mathds{1}_\mathcal{C}(\mathbf{z})\mathds{1}_\mathcal{C}(\mathbf{x}+\mathbf{z}) =\mathds{1}_\mathcal{C}(\mathbf{z})\mathds{1}_\mathcal{C}(\mathbf{x})$, and hence $f_\mathcal{C}$ evaluates to simply $ \mathds{1}_\mathcal{C}$. }
\[
f_\mathcal{C} = \frac{2^n}{|\mathcal{C}|}\mathds{1}_\mathcal{C}\star \mathds{1}_\mathcal{C}.
\]
We claim that $f_\mathcal{C}$ is a feasible solution for $\mathsf{Del}(n,d)$, with the objective function (Obj) evaluating to $|\mathcal{C}|$. Indeed, observe that (C1) is trivially satisfied, by the definition of the convolution operator. Further, since $\widehat{f_\mathcal{C}} = \frac{2^n}{|\mathcal{C}|}\cdot \widehat{\mathds{1}_\mathcal{C}}^2$, it holds that (C2) is satisfied as well. Next, note that since $\mathcal{C}$ is such that $d(\mathcal{C})\geq d$, it holds that $\mathds{1}_\mathcal{C}(\mathbf{x}+\mathbf{z}) = 0$, for all $\mathbf{z}\in \mathcal{C}$ and any $\mathbf{x}$ such that $1\leq w(\mathbf{x})\leq d-1$. In other words, we have that $\mathds{1}_\mathcal{C}(\mathbf{z})\cdot \mathds{1}_\mathcal{C}(\mathbf{x}+\mathbf{z}) = 0$, for all $\mathbf{z}\in \{0,1\}^n$, if $1\leq w(\mathbf{x})\leq d-1$. Hence, (C3) is also true. Finally, observe that
\begin{align*}
	f_\mathcal{C}(0^n)&= \frac{1}{|\mathcal{C}|}\sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{C}(\mathbf{z})\cdot \mathds{1}_\mathcal{C}(\mathbf{z})\\
	&= \frac{1}{|\mathcal{C}|}\sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{C}(\mathbf{z}) = 1,
\end{align*}
thereby satisfying (C4) also. Now, it holds that the objective value of $f_\mathcal{C}$, which is $\sum_{\mathbf{x}\in \{0,1\}^n} f_\mathcal{C}(\mathbf{x})$, is given by
\begin{align}
	\sum_{\mathbf{x}\in \{0,1\}^n} f_\mathcal{C}(\mathbf{x})&= \frac{1}{|\mathcal{C}|}\sum_{\mathbf{x}\in \{0,1\}^n} \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{C}(\mathbf{z})\cdot \mathds{1}_\mathcal{C}(\mathbf{x}+\mathbf{z}) \notag\\
	&= \frac{1}{|\mathcal{C}|}\sum_{\mathbf{z}\in \{0,1\}^n}\mathds{1}_\mathcal{C}(\mathbf{z}) \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_\mathcal{C}(\mathbf{x}+\mathbf{z}) \notag\\
	&= \frac{|\mathcal{C}|^2}{|\mathcal{C}|} = |\mathcal{C}|. \label{eq:temp1}
\end{align}
Hence, it holds that the optimal value of $\mathsf{Del}(n,d)$, is an upper bound on $|\mathcal{C}|$, for all block codes $\mathcal{C}$ of blocklength $n$ and minimum distance at least $d$, and therefore also an upper bound on $A(n,d)$. We refer the reader to \cite{delsarte, mrrw, friedman, sam1, coregliano, linial1} and the references therein for a more detailed treatment of linear programming-based upper bounds on the sizes of block codes and linear codes, and for the derivation of analytical upper bounds via the dual LP or using modern Fourier-theoretic or expander graph-based arguments.

Our LP, which we call $\mathsf{Del}(n,d;\mathcal{A})$, is but a small modification of $\mathsf{Del}(n,d)$, to take into account the fact that all codewords of the code of minimum distance at least $d$, whose size we are attempting to bound, must also lie in the set $\mathcal{A}\subseteq \mathbb{F}_2^n$.
\begin{center}
%	\begin{mybox}[colback=white, width = 0.75\linewidth]{$1,2$}
%		This is my box.
%	\end{mybox}
\begin{tcolorbox}[title={\center $\mathsf{Del}(n,d;\mathcal{A})$}, title filled = false, width = 0.6\linewidth]
	\begin{align}
		&\underset{f:\ \{0,1\}^n\to \mathbb{R}}{\text{maximize}}\quad \sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x}) \tag{Obj$^\prime$}\\
		&\text{subject to:} \notag\\
		&\ \ f(\mathbf{x})\geq 0,\ \forall\ \mathbf{x}\in \{0,1\}^n, \tag{D1}\\
		&\ \ \widehat{f}(\mathbf{s})\geq 0,\ \forall\ \mathbf{s}\in \{0,1\}^n, \tag{D2}\\
		&\ \ f(\mathbf{x}) = 0,\ \text{if $1\leq w(\mathbf{x})\leq d-1$}, \tag{D3}\\
		&\ \ f(0^n)\leq \text{val}(\mathsf{Del}(n,d)), \tag{D4}\\
		&\ \ f(\mathbf{x})\leq 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}),\ \forall\ \mathbf{x}\in \{0,1\}^n. \tag{D5}
	\end{align}
\end{tcolorbox}
\end{center}
Like in the case with $\mathsf{Del}(n,d)$, we produce a feasible solution for $\mathsf{Del}(n,d;\mathcal{A})$, and claim that val$(\mathsf{Del}(n,d;\mathcal{A}))$ is at least $(A(n,d;\mathcal{A}))^2$ (note the difference with $\mathsf{Del}(n,d)$, whose value is at least $A(n,d)$). To this end, let $\mathcal{C}_\mathcal{A}$ be any length-$n$ constrained code, with $d(\mathcal{C}_\mathcal{A})\geq d$, such that all codewords in $\mathcal{C}_\mathcal{A}$ lie in $\mathcal{A}$. Observe that we can write $\mathcal{C}_\mathcal{A}$ as $\mathcal{C}\cap \mathcal{A}$, for some block (not necessarily constrained) code $\mathcal{C}$, with $d(\mathcal{C})\geq d$. Thus, an upper bound on $\max\limits_{\substack{\mathcal{C}:\ d(\mathcal{C})\geq d}}|\mathcal{C}\cap \mathcal{A}|$ serves as an upper bound on (and in fact, equals) $A(n,d;\mathcal{A})$. 

Let $\mathds{1}_\mathcal{C}$ be the indicator function of a block code $\mathcal{C}$ as above, and let $\mathds{1}_\mathcal{A}$ be the indicator function of the constraint. We define
\[
f_{\mathcal{C},\mathcal{A}} = 2^n\cdot (\mathds{1}_\mathcal{C}\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{C}\mathds{1}_\mathcal{A}),
\]
and claim that $f_{\mathcal{C},\mathcal{A}}$ is a feasible solution for $\mathsf{Del}(n,d;\mathcal{A})$, with the objective function (Obj$^\prime$) evaluating to $|\mathcal{C}\cap \mathcal{A}|^2$. To see this, note that the LP constraints (D1)--(D3) are satisfied for the same reasons as why $f_\mathcal{C}$ satisfied (C1)--(C3) in $\mathsf{Del}(n,d)$. Furthermore,
\begin{align*}
	f_{\mathcal{C},\mathcal{A}}(0^n) &= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_{\mathcal{C}\cap \mathcal{A}}(\mathbf{z})\\
	&= |\mathcal{C}\cap \mathcal{A}|\leq |\mathcal{C}|\leq \text{val}(\mathsf{Del}(n,d)),
\end{align*}
since $\mathcal{C}$ is a block code of distance at least $d$. Hence, (D4) is satisfied by $f_{\mathcal{C},\mathcal{A}}$. Finally, observe that for any $\mathbf{x}\in \{0,1\}^n$, 
\begin{align*}
	f_{\mathcal{C},\mathcal{A}}(\mathbf{x}) &= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_{\mathcal{C}}\mathds{1}_{\mathcal{A}}(\mathbf{z})\cdot \mathds{1}_\mathcal{C}(\mathbf{x}+\mathbf{z})\mathds{1}_\mathcal{A}(\mathbf{x}+\mathbf{z})\\
	&\leq \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_{\mathcal{A}}(\mathbf{z})\cdot \mathds{1}_\mathcal{A}(\mathbf{x}+\mathbf{z}) = 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}),
\end{align*}
showing that (D5) also holds. Now, note that val$(f_{\mathcal{C},\mathcal{A}})$, which is $\sum_{\mathbf{x}\in \{0,1\}^n} f_{\mathcal{C},\mathcal{A}}(\mathbf{x})$, equals $|\mathcal{C}\cap \mathcal{A}|^2$, by calculations as in \eqref{eq:temp1}. Hence, we have that val$(\mathsf{Del}(n,d;\mathcal{A}))\geq |\mathcal{C}\cap \mathcal{A}|^2$, for any $\mathcal{C}$ with minimum distance at least $d$. Therefore, it holds that val$(\mathsf{Del}(n,d;\mathcal{A}))\geq (A(n,d;\mathcal{A}))^2$, or, that $A(n,d;\mathcal{A})\leq (\text{val}(\mathsf{Del}(n,d;\mathcal{A})))^{1/2}$.

We now discuss a couple of observations about $\mathsf{Del}(n,d;\mathcal{A})$. Firstly, note that by (D5), we have that for any feasible solution $f$ of $\mathsf{Del}(n,d;\mathcal{A})$, it holds that the objective value
\begin{align*}
	\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x})&\leq \sum_{\mathbf{x}\in \{0,1\}^n} \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\mathbf{z})\cdot \mathds{1}_\mathcal{A}(\mathbf{x}+\mathbf{z})\\
	&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\mathbf{z}) \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\mathbf{x}+\mathbf{z})
	= |\mathcal{A}|^2.
\end{align*}
Therefore, we have that our upper bound that is  $(\text{val}(\mathsf{Del}(n,d;\mathcal{A})))^{1/2}$ is less than or equal to $|\mathcal{A}|$, which is the total number of constrained sequences of length $n$.

Second, from the proof of Proposition 1 in \cite{linial1}, we obtain that for any feasible solution $f$ of $\mathsf{Del}(n,d;\mathcal{A})$, for all $\mathbf{x}\in \{0,1\}^n$, it holds that $f(\mathbf{x})\leq f(0^n)\leq \text{val}(\mathsf{Del}(n,d))$. Hence, we have that the objective value of $f$, for any feasible $f$, obeys
\[
	\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x})\leq \left({n\choose \geq d}+1\right)\cdot \text{val}(\mathsf{Del}(n,d)),
\]
since $f(\mathbf{x}) = 0$, if $1\leq \text{wt}(\mathbf{x})\leq d-1$, where we define ${n\choose \geq d}:= \sum_{i=d}^n {n\choose i}$. Therefore, we have that $(\text{val}(\mathsf{Del}(n,d;\mathcal{A})))^{1/2}\leq \left({n\choose \geq d}+1\right)^{1/2}\cdot (\text{val}(\mathsf{Del}(n,d)))^{1/2}$. Moreover, for most constraints that we ran either $\mathsf{Del}(n,d;\mathcal{A})$ or the equivalent symmetrized LP $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$ (see Section \ref{sec:sym}) on, the value of the LP came out to be strictly less than $\text{val}(\mathsf{Del}(n,d))$ (see also the remark after the proof of Lemma \ref{lem:dual}).

Next, we derive an upper bound on the optimal value val$(\mathsf{Del}(n,d;\mathcal{A}))$ of our LP, in the following lemma that is essentially a formulation of the dual LP. While we do not apply Lemma \ref{lem:dual} elsewhere in this paper, we believe that it will serve useful in the derivation of asymptotic (as the blocklength goes to infinity) upper bounds on the rate-distance tradeoff for constrained codes. We abbreviate $	\text{val}(\mathsf{Del}(n,d))$ as $v$ and $\text{val}(\mathsf{Del}(n,d;\mathcal{A}))$ as $v_\mathcal{A}$.

\begin{lemma}
	\label{lem:dual}
	Let $\beta: \{0,1\}^n \to \mathbb{R}$ be a function that satisfies $\widehat{\beta}(\mathbf{s})\geq 0$, for all $\mathbf{s}\in \{0,1\}^n$, and $\sum_{\mathbf{x}}\beta(\mathbf{x}) = 1$. Then,
	\[
	v_\mathcal{A}\leq 2^n\cdot \left[\beta(0^n)\cdot \min\{v,|\mathcal{A}|\}+2^n\cdot \sum_{\mathbf{x}:\ w(\mathbf{x})\geq d} \beta(\mathbf{x})\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x})\right].
	\]
\end{lemma}
\begin{proof}
	Consider any function $\lambda: \{0,1\}^n\to [0,\infty)$. Now, observe that for any feasible solution $f$ of $\mathsf{Del}(n,d;\mathcal{A})$, we have that
	\begin{align*}
		\lambda(0^n)\cdot \widehat{f}(0^n)&\stackrel{(a)}{\leq} \sum_{\mathbf{x}\in \{0,1\}^n}\lambda(\mathbf{x})\cdot \widehat{f}(\mathbf{x})\\
		&\stackrel{(b)}{=} 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\lambda}(\mathbf{s})\cdot \frac{f(\mathbf{s})}{2^n}\\
		&\stackrel{(c)}{=} \sum_{\substack{\mathbf{s}:\ \mathbf{s}\ =\ 0^n\text{ or }\\w(\mathbf{s})\geq d}} \widehat{\lambda}(\mathbf{s})\cdot f(\mathbf{s})\\
		&\stackrel{(d)}{\leq} \widehat{\lambda}(0^n)\cdot \min\{v,|\mathcal{A}|\}+2^n\cdot \sum_{\mathbf{s}:\ w(\mathbf{s})\geq d} \widehat{\lambda}(\mathbf{s})\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{s}),
	\end{align*}
where (a) holds since $\lambda, \widehat{f}\geq 0$, (b) holds by an application of Plancherel's Theorem, along with the fact that $\widehat{(\widehat{f})} = 2^{-n}\cdot f$. Next, (c) is true since $f$ satisfies (D3) and (d) holds since $f$ satisfies (D4) and (D5), and since $2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(0^n) = |\mathcal{A}|$.

Moreover, we have that val$(f) = \sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x}) = 2^n\cdot \widehat{f}(0^n)$, and that $\lambda(0^n) = \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\lambda}(\mathbf{s})$, by the definition of the Fourier transform. Putting everything together, we obtain that for any feasible $f$ of $\mathsf{Del}(n,d;\mathcal{A})$, it holds that
\[
\text{val}(f)\leq \frac{2^n}{\sum_\mathbf{s} \widehat{\lambda}(\mathbf{s})}\cdot \left[\widehat{\lambda}(0^n)\cdot \min\{v,|\mathcal{A}|\}+2^n\cdot \sum_{\mathbf{s}:\ w(\mathbf{s})\geq d} \widehat{\lambda}(\mathbf{s})\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{s})\right].
\]
Finally, by substituting $\beta$ as $\widehat{\lambda}$ and ensuring that $\sum_\mathbf{x} \widehat{\beta}(\mathbf{x}) = 1$, we obtain the thesis of the lemma.
\end{proof}
\begin{remark}
	As a simple corollary of the above lemma, note that we can pick $\beta(\mathbf{x}) = 2^{-n}$, for all $\mathbf{x}\in \{0,1\}^n$, so that $\widehat{\beta}(\mathbf{s}) = 2^{-2n}$, if $\mathbf{s} = 0^n$ and $\widehat{\beta}(\mathbf{s}) = 0$, for $\mathbf{s}\neq 0^n$. Then, we obtain that
	\begin{align*}
		v_\mathcal{A}&\leq \min\{v,|\mathcal{A}|\}+2^{-n}\cdot \sum_{\mathbf{x}:\ w(\mathbf{x})\geq d} \sum_{\mathbf{z}} \mathds{1}_\mathcal{A}(\mathbf{z})\cdot \mathds{1}_\mathcal{A}(\mathbf{x}+\mathbf{z})\\
		&\leq \min\{v,|\mathcal{A}|\}+\frac{|\mathcal{A}|^2}{2^n}.
	\end{align*}
Hence, if $|\mathcal{A}|\leq 2^{n/2}$, we get that $v_{\mathcal{A}}\leq v+1$.
\end{remark}
\subsection{Numerical Trials}
In what follows, we discuss some numerical results we obtained by running $\mathsf{Del}(n,d;\mathcal{A})$, for select constraints. 
\subsubsection{$(d,\infty)$-RLL constraint}

We first consider the so-called $(\ell,\infty)$-runlength limited (RLL) constraint. This constraint mandates that there be at least $\ell$ $0$s between every pair of successive $1$s in the binary input sequence, where $\ell\geq 1$. For example, when $\ell=3$, the sequence $10001000010$ respects the $(3,\infty)$-RLL constraint, but the sequence $10100010$, does not. It can also be checked that the $(1,\infty)$-RLL constraint is the same as a ``no-consecutive-ones'' constraint. Clearly, here, $\mathcal{A}$ is the set of all binary sequences of length $n$ that respect the $(d,\infty)$-RLL constraint. The $(\ell,\infty)$-RLL constraint is a special case of the $(\ell,h)$-RLL constraint (we avoid using the more common notation that is $(d,k)$-RLL for such constraints, in order to avoid confusion with existing notation), which admits only binary sequences in which successive $1$s are separated by at least $\ell$ $0$s, and the length of any run of $0$s is at most $h$. Such constraints find application in magnetic and optical recording systems, where the $(\ell,\infty)$-RLL constraint on the data sequence (with the bit $1$ corresponding to a voltage peak of high amplitude and the bit $0$ corresponding to no peak) ensures that successive $1$s are spaced far enough apart, so that there is little inter-symbol interference (ISI) between the voltage responses corresponding to the magnetic transitions. Reference \cite{Immink2} contains many examples of $(\ell,h)$-RLL codes used in practice in magnetic storage and recording. More recently, $(\ell,h)$-RLL input constrained sequences have also been investigated for joint energy and information transfer performance \cite{infoenergy}. We let $S_{(\ell,\infty)}$ denote the set of $(\ell,\infty)$-RLL constrained binary words of length $n$.

Table \ref{tab1} (resp. Table \ref{tab2}) shows comparisons between the upper bounds on $A(n,d;S_{(1,\infty)})$ (resp. $A(n,d;S_{(2,\infty)})$), obtained using our  $\mathsf{Del}(n,d;S_{(1,\infty)})$ LP (resp. $\mathsf{Del}(n,d;S_{(2,\infty)})$ LP) with the generalized sphere packing bound of \cite{cullina} and \cite{fazeli}, when $n=10$, and for varying values of the minimum distance $d$. We also compare these upper bounds with the optimal value of $\mathsf{Del}(n,d)$, since this is a trivial upper bound on $A(n,d;\mathcal{A})$, for any $\mathcal{A}\subseteq \{0,1\}^n$. Note that, from the numerical trials, for certain values of $d$, the generalized sphere-packing bound returns a value that is larger (and hence worse) than the value of $\mathsf{Del}(n,d)$, whereas the optimal value of our $\mathsf{Del}(n,d;\mathcal{A})$ LP is uniformly bounded above by $\mathsf{Del}(n,d)$.

\begin{table}[t!]
	\centering
	\begin{tabular}{||c || c || c || c ||} 
		\hline
		 $d$ & $\mathsf{Del}(n,d;S_{(1,\infty)})$& $\mathsf{GenSph}(n,d;S_{(1,\infty)})$ & $\mathsf{Del}(n,d)$\\ [0.5ex] 
		\hline\hline
		$2$ & $128.557$ & $144$ & $512$\\ 
		\hline
		$3$ & $74.762$ & $111$ & $85.333$\\ 
		\hline
		$4$ & $42.048$ & $111$ & $42.667$\\ 
		\hline
		$5$ & $12$ & $63$ & $12$\\ 
		\hline
		$6$ & $6$ & $63$ & $6$\\ 
		\hline
		$7$ & $3.2$ & $26$ & $3.2$\\ 
		\hline
	\end{tabular}
	\caption{Table of values of optimal values of the $\mathsf{Del}(n,d;S_{(1,\infty)})$ LP, the generalized sphere packing bound LP $\mathsf{GenSph}(n,d;S_{(1,\infty)})$ in \cite{cullina} and \cite{fazeli}, and the $\mathsf{Del}(n,d)$ LP, for $n=10$ and varying values of $d$.}
	\label{tab1}
\end{table}

\begin{table}[t!]
	\centering
	\begin{tabular}{||c || c || c || c ||} 
		\hline
		$d$ & $\mathsf{Del}(n,d;S_{(2,\infty)})$ & $\mathsf{GenSph}(n,d;S_{(2,\infty)})$ & $\mathsf{Del}(n,d)$\\ [0.5ex] 
		\hline\hline
		$2$ & $49.578$ & $60$ & $512$\\ 
		\hline
		$3$ & $32.075$ & $46.5$ & $85.333$\\ 
		\hline
		$4$ & $21.721$ & $46.5$ & $42.667$\\ 
		\hline
		$5$ & $7.856$ & $34$ & $12$\\ 
		\hline
		$6$ & $4.899$ & $34$ & $6$\\ 
		\hline
		$7$ & $2.529$ & $19$ & $3.2$\\ 
		\hline
	\end{tabular}
	\caption{Table of values of optimal values of the $\mathsf{Del}(n,d;S_{(2,\infty)})$ LP, the generalized sphere packing bound LP $\mathsf{GenSph}(n,d;S_{(2,\infty)})$, and the $\mathsf{Del}(n,d)$ LP, for $n=10$ and varying values of $d$.}
	\label{tab2}
\end{table}

==> odd.tex <==
\label{sec:odd}
In this section, we work with the so-called odd constraint on binary sequences, which mandates that the number of $0$s between successive $1$s is odd. Initially, we shall impose the additional restriction that the number of $0$s until the occurence of the first $1$ in the sequence (also known as the length of the ``leading'' run of $0$s) and the number of $0$s after the occurence of the last $1$ in the sequence (also known as the length of the ``trailing'' run of $0$s) also be odd. In other words, we require that the lengths of all runs of $0$s in the binary sequence be odd. We also use the convention that the all-zeros word respects the constraint. We let $S_{\text{o}^\star}^{(n)}$ be the set of such constrained sequences of length $n$, and drop the superscript `$(n)$' when it is clear from the context. It can be checked that if $n$ is even, then there are no sequences that lie in $S_{\text{o}^\star}^{(n)}$. We hence assume that $n$ is odd.

It is known (see, for example, \cite{odd1} and \cite{odd2}) that in certain types of magneto-optical recording systems, it is detrimental to have odd lengths of $0$ runs, and one may hence be interested in eliminating sequences all of whose $0$ runs have odd length. Our interest may therefore be in using linear codes (over noisy channels, say) whose subcodes that lie in $S_{\text{o}^\star}$ are of small size. To this end, it is essential that we obtain estimates of the sizes of such constrained subcodes of known linear codes.

Now, we first observe that the binary sequences that lie in $S_{\text{o}^\star}$ are supported exclusively on even coordinate positions. It is thus true that the set $S_{\text{o}^\star}$ is by itself a subspace of $\mathbb{F}_2^n$, of dimension $\left\lfloor \frac{n}{2}\right \rfloor$. We let $S_{\text{o}^\star}^{\perp}$ denote the orthogonal complement (or dual) of $S_{\text{o}^\star}$, which is set of length-$n$ binary sequences that are supported exclusively on odd coordinates, with the convention that the all-zeros sequence is present in $S_{\text{o}^\star}^{\perp}$. By using the arguments in the proof of Theorem \ref{thm:lincount}, we obtain the following lemma:
\begin{lemma}
	\label{lem:fcoeffo}
	For $\mathbf{s}\in \{0,1\}^n$, where $n$ is odd, it holds that
	\[
	\widehat{\mathds{1}_{S_{\text{o}^\star}}}(\mathbf{s}) = 2^{\left\lfloor \frac{n}{2}\right \rfloor - n}\cdot \mathds{1}_{S_{\text{o}^\star}^{\perp}}(\mathbf{s}).
	\]
\end{lemma}
\begin{proof}
	The proof is based on the observation that $S_{\text{o}^\star}$ is a subspace  of $\mathbb{F}_2^n$ (or equivalently, a linear code). From \eqref{eq:Ccoeff} and the fact that $|S_{\text{o}^\star}| = 2^{\left\lfloor \frac{n}{2}\right \rfloor}$, we obtain the required result.
\end{proof}
We shall now use Lemma \ref{lem:fcoeffo} and Theorem \ref{thm:lincount} to calculate the number of codewords in the $[2^m-1,2^m-m-1]$ binary Hamming code, for $m\geq 1$, that lie in $S_{\text{o}^\star}$. We once again use the coordinate ordering given in Section \ref{sec:prelim}.
\begin{corollary}
	For $m\geq 1$ and for $\mathcal{C}$ being the $[2^m-1,2^m-m-1]$ binary Hamming code, we have that $N(\mathcal{C};S_{\text{o}^\star}) = 2^{\left\lfloor \frac{2^m-1}{2}\right \rfloor -m}$.
\end{corollary}
\begin{proof}
	The dual code $\mathcal{C}^\perp$ of the binary Hamming code is the $[2^m-1,m]$ binary simplex code, a generator matrix for which is $H_{\text{Ham}}$. We once again use the fact that any codeword $\mathbf{s}\in \mathcal{C}^\perp$ is such that $w(\mathbf{s}) = 2^{m-1}$. Note that the only word that is of weight $2^{m-1}$, and is supported entirely on even coordinates, is the word $\mathbf{s}^\star = 0101\ldots10$, consisting of alternating $1$s and $0$s. However, $\mathbf{s}^\star \notin \mathcal{C}^\perp$. Indeed, by standard arguments such as those made in the proof of Corollary \ref{cor:s2hamming} that associate the rows of $H_{\text{Ham}}$ with evaluation vectors of Boolean polynomials, it can be checked that the last row of $H_{\text{Ham}}$ equals the vector $1010\ldots01$, which implies that $1010\ldots01\in \mathcal{C}^\perp$. However, since the all-ones vector $1^{2^m-1}\notin \mathcal{C}^\perp$, we get that $\mathbf{s}^\star \notin \mathcal{C}^\perp$.
	
	Hence, the only codeword in $\mathbf{s}\in\mathcal{C}^\perp$ whose Fourier coefficient $\widehat{\mathds{1}_{S_{\text{o}^\star}}}(\mathbf{s})$ takes a nonzero value is (see Lemma \ref{lem:fcoeffo}) the all-zeros word $0^{2^m-1}$. Therefore, we get that
	\begin{align*}
		N(\mathcal{C},S_{\text{o}^\star}) &= |\mathcal{C}|\cdot  \sum_{\mathbf{s}\in \mathcal{C}^\perp} \widehat{\mathds{1}_{S_{\text{o}^\star}}}(\mathbf{s})\\
		&= 2^{2^m-1-m}\cdot  2^{\left\lfloor \frac{2^m-1}{2}\right \rfloor - (2^m-1)} = 2^{\left\lfloor \frac{2^m-1}{2}\right \rfloor -m}.
	\end{align*}
\end{proof}
Observe that although the number of constrained codewords $N(\mathcal{C},S_{\text{o}^\star})$ in the corollary above is much smaller than the number of words, $2^{\left\lfloor \frac{2^m-1}{2}\right \rfloor}$ in $S_{\text{o}^\star}$ of blocklength $2^m-1$, the rate of the largest constrained subcode $\mathcal{C}_{\text{o}^\star}$ of the binary Hamming code $\mathcal{C}$, in the limit as the blocklength goes to infinity, is still equal to the noiseless capacity $C_0(S_{\text{o}^\star})$ of the odd constraint. Indeed, we have that
\begin{align*}
	\liminf_{m\to \infty}\text{rate}\left(\mathcal{C}_{\text{o}^\star}\right) &= \liminf_{m\to \infty} \frac{\log_2 N(\mathcal{C};S_{\text{o}^\star})}{2^m}\\
	&= \lim_{m\to \infty} \frac{\left\lfloor \frac{2^m-1}{2}\right \rfloor -m}{2^m}\\
	&= \frac12 = \lim_{m\to \infty} \frac{\left \lvert S_{\text{o}^\star}^{(2^m)}\right \rvert}{2^m}.
\end{align*}

Next, in the odd constraint, we shall remove the condition that the lengths of the first and last runs of $0$s must also be odd. In particular, we define the (constrained) set $S_\text{o}^{(n)}$ (or, simply, $S_\text{o}$) to be the set of all binary sequences such that the number of $0$s between successive $1$s is odd. We again use the convention that the all-zeros sequence is present in $S_\text{o}$. In what follows, we shall only concern ourselves with the setting where the blocklength $n$ is even. The case where $n$ is odd can be handled similarly. We put down a lemma on the Fourier coefficents of the indicator function that a codeword belongs to $S_\text{o}$.
\begin{lemma}
	For $\mathbf{s}\in \{0,1\}^n$, with $n$ being even, we have that
	\[
	\widehat{\mathds{1}_{S_{\text{o}}}}(\mathbf{s}) = \begin{cases}
		\frac{2^{\frac{n}{2}+1}-1}{2^n},\ \text{if $\mathbf{s} = 0^n$},\\
		\frac{2^{\frac{n}{2}}-1}{2^n},\ \text{if $\mathbf{s}\in S_\text{o} \setminus \{0^n\}$},\\
		-2^{-n},\ \text{otherwise.}
	\end{cases}
	\]
\end{lemma}
\begin{proof}
	First, we note that when $\mathbf{s} = 0^n$, the Fourier coefficient
	\begin{align*}
		\widehat{\mathds{1}_{S_{\text{o}}}}(0^n) &= \frac{1}{2^n}\cdot \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_{S_{\text{o}}}(\mathbf{x})\cdot (-1)^{\mathbf{x}\cdot 0^n}\\
		&= \frac{1}{2^n}\cdot \sum_{\mathbf{x}\in S_{\text{o}}} 1 = \frac{|S_{\text{o}}|}{2^n} = \frac{2^{\frac{n}{2}+1}-1}{2^n},
	\end{align*}
where the last equality holds by the following argument: let supp$_\text{e}$ and supp$_\text{o}$ denote the set of binary words supported on even and odd coordinates, respectively, with the convention that $0^n\notin \text{supp}_\text{e}\cup \text{supp}_\text{o}$, but $0^n\in S_\text{o}$. Then, clearly, we have that $|S_\text{o}| = |\text{supp}_\text{e}|+|\text{supp}_\text{o}|+1 = 2\cdot (2^{\frac{n}{2}}-1)+1 = 2^{\frac{n}{2}+1}-1$.

Next, consider the case when $\mathbf{s}\in S_\text{o}\setminus \{0^n\}$. This implies that $\mathbf{s}\in \text{supp}_\text{o}$ or $\mathbf{s}\in \text{supp}_\text{e}$. Suppose that $\mathbf{s}\in \text{supp}_\text{o}$. Then, observe that
\begin{align}
	\widehat{\mathds{1}_{S_{\text{o}}}}(\mathbf{s}) &= \frac{1}{2^n}\cdot \sum_{\mathbf{x}\in S_\text{o}} (-1)^{\mathbf{x}\cdot \mathbf{s}} \notag\\
	&= \frac{1}{2^n}\cdot\left(\sum_{\mathbf{x}\in S_\text{o}\cap \text{supp}_\text{e}} 1 + \sum_{\mathbf{x}\in (S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\}} (-1)^{\mathbf{x}\cdot \mathbf{s}}\right) \label{eq:inter6},
\end{align}
where the last equality holds since the all words supported on even coordinates are orthogonal to words supported on odd coordinates. Moreover, since $(S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\} = \text{supp}_\text{o}\cup \{0^n\}$ forms a vector space of dimension $\frac{n}{2}$, it can be verified that $\sum\limits_{\mathbf{x}\in (S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\}} (-1)^{\mathbf{x}\cdot \mathbf{s}} = \sum\limits_{\mathbf{x}\in (S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\}} (-1)^{w_\mathbf{s}(\mathbf{x})} = 0$, since the number of words $\mathbf{x}\in (S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\}$ such that $w_\mathbf{s}(\mathbf{x})$ is even equals the number such that $w_\mathbf{s}(\mathbf{x})$ is odd. Plugging back in \eqref{eq:inter6}, we obtain that
\[
\widehat{\mathds{1}_{S_{\text{o}}}}(\mathbf{s}) = \frac{|\text{supp}_\text{e}|}{2^n} = \frac{2^{\frac{n}{2}}-1}{2^n}, \ \text{if $\mathbf{s}\in S_\text{o}\setminus \{0^n\}$ and supp$(\mathbf{s})\subseteq \text{supp}_\text{o}$}.
\]
By arguing similarly, we also get that when $\mathbf{s}\in S_\text{o}\setminus \{0^n\}$ and supp$(\mathbf{s})\subseteq \text{supp}_\text{e}$, the Fourier coefficient $\widehat{\mathds{1}_{S_{\text{o}}}}(\mathbf{s})$ equals $\frac{2^{\frac{n}{2}}-1}{2^n}$. 

Finally, we take up the case when $\mathbf{s}\notin S_\text{o}\cup\{0^n\}$. For any vector $\mathbf{y}\in \{0,1\}^n$, we define the vectors $\mathbf{y}_\text{e} := \left(y_i:\ i\text{ is even}\right)\in \{0,1\}^{n/2}$ and $\mathbf{y}_\text{o} := \left(y_i:\ i\text{ is odd}\right)\in \{0,1\}^{n/2}$ to be the substrings of the word $\mathbf{y}$, supported on even and odd coordinate positions, respectively. Then,
\begin{align*}
	\widehat{\mathds{1}_{S_{\text{o}}}}(\mathbf{s}) &= \frac{1}{2^n}\cdot \sum_{\mathbf{x}\in S_\text{o}} (-1)^{\mathbf{x}\cdot \mathbf{s}} \notag\\
	&= \frac{1}{2^n}\cdot\left(\sum_{\mathbf{x}\in S_\text{o}\cap \text{supp}_\text{e}} (-1)^{\mathbf{x}\cdot \mathbf{s}} + \sum_{\mathbf{x}\in (S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\}} (-1)^{\mathbf{x}\cdot \mathbf{s}}\right)\\
	&= \frac{1}{2^n}\cdot\left(\sum_{\mathbf{x}\in S_\text{o}\cap \text{supp}_\text{e}} (-1)^{\mathbf{x}_\text{e}\cdot \mathbf{s}_\text{e}}\cdot (-1)^{\mathbf{x}_\text{o}\cdot \mathbf{s}_\text{o}} + \sum_{\mathbf{x}\in (S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\}} (-1)^{\mathbf{x}_\text{e}\cdot \mathbf{s}_\text{e}}\cdot (-1)^{\mathbf{x}_\text{o}\cdot \mathbf{s}_\text{o}}\right)\\
	&= \frac{1}{2^n}\cdot\left(\sum_{\mathbf{x}\in S_\text{o}\cap \text{supp}_\text{e}} (-1)^{\mathbf{x}_\text{e}\cdot \mathbf{s}_\text{e}} + \sum_{\mathbf{x}\in (S_\text{o}\cap \text{supp}_\text{o})\cup \{0^n\}} (-1)^{\mathbf{x}_\text{o}\cdot \mathbf{s}_\text{o}}\right) = \frac{1}{2^n}\cdot (-1+0) = -2^{-n},
\end{align*}
where the last equality holds by similar arguments as previously.
\end{proof}
%We now apply Theorem \ref{thm:lincount} and Lemma \ref{lem:fcoeffo} to numerically calculate the number of codewords in Reed-Muller codes RM$(m,r)$ that lie in $S_\text{o}$, for varying values of $m\geq 1$ and $r\leq m$. As is usual, we assume that the coordinates of the RM codes are ordered according to the standard lexicographic ordering. We once again note the computational savings obtained by applying Theorem \ref{thm:lincount} to count the number of constrained codewords in RM codes whose rate is larger than half. Our results are listed in Table \ref{tab:rmo}. (\textbf{Change this to just remark that the odd constrained codewords in RM$(m,r)$ are codewords of the form Eval$(x_m\cdot h)$ and Eval$((1+x_m)\cdot h)$.})
While it is possible to use Lemma \ref{lem:fcoeffo} and Theorem \ref{thm:lincount} to count the number of codewords in Reed-Muller codes RM$(m,r)$ that lie in $S_\text{o}$, for varying values of $m\geq 1$ and $r\leq m$, we discuss here a direct argument that enables us to arrive at $N(\text{RM}(m,r);S_\text{o})$. We write a codeword of RM$(m,r)$ as $\mathbf{c} = (c_1,c_2,\ldots,c_{2^m})$, with $\mathbf{c} = (f(\mathbf{B}_m(0)),f(\mathbf{B}_m(1)),\ldots,f(\mathbf{B}_m(2^m-1)))$, for some Boolean polynomial $f$ such that deg$(f)\leq r$. In such a case, we also use the represent $\mathbf{c}$ as Eval$(f)$. Recall that the coordinates of the RM code can also be written as $m$-tuples $(x_1,\ldots,x_m)\in \{0,1\}^m$ that follow the lexicographic ordering.  Now, observe that for $m\geq 1$, it holds that Eval$(x_m)$ has $1$s in even coordinates $i \in [2^m]$ and $0$s in odd coordinates. Similarly, for $m\geq 1$, it holds that Eval$(1+x_m)$ has $1$s in odd coordinates $i \in [2^m]$ and $0$s in even coordinates. It can be thus be argued that for any codeword $\mathbf{c}\in \text{RM}(m,r)$ such that $\mathbf{c}\in S_\text{o}$, it must be that either supp$(\mathbf{c})$ lies entirely within the odd or entirely within the even coordinate positions, or $\mathbf{c} = 0^{2^m}$. Hence, it must be the case that $\mathbf{c} = \text{Eval}(x_m\cdot h(x_1,\ldots,x_{m-1}))$ or $\mathbf{c} = \text{Eval}((1+x_m)\cdot h(x_1,\ldots,x_{m-1}))$, for some polynomial $h$ in the variables $x_1,\ldots,x_{m-1}$ such that deg$(h)\leq r-1$, or that $\mathbf{c} = 0^{2^m}$. Therefore, we have that 
\begin{align*}
	N(\text{RM}(m,r);S_\text{o})&\stackrel{(a)}{=} 2\cdot|\{h: h\text{ is a non-zero polynomial in $m-1$ variables with deg}(h)\leq r-1\}|+1\\
	&= 2\cdot\left(2^{{m-1\choose \leq r-1}}-1\right)+1 = 2^{{m-1\choose \leq r-1}+1}-1,
\end{align*}
where in (a) above, the additive factor of `$+1$' accounts for the all-zeros word.
%\begin{table}[t!]
%	\centering
%	\begin{tabular}{||c || c||} 
%		\hline
%		$(m,r)$ & $N(\text{RM}(m,r);S_\text{o})$\\ [0.5ex] 
%		\hline\hline
%		$(4,2)$ & $31$\\ 
%		\hline
%		$(4,3)$ & $255$\\ 
%		\hline
%		$(5,2)$ & 63\\
%		\hline
%		$(5,3)$ & $4095$\\
%		\hline
%		$(6,3)$ & $131071$\\
%		\hline
%		$(6,4)$ & $1.342\times 10^8$\\
%		\hline
%		$(7,5)$ & $2.882\times 10^{17}$\\
%		\hline
%	\end{tabular}
%	\caption{Table of values of $N(\text{RM}(m,r);S_\text{o})$, for select parameters $m$ and $r$}
%	\label{tab:rmo}
%\end{table}

We note, however, that the structure of the Fourier coefficients in Lemma \ref{lem:fcoeffo} along with Theorem \ref{thm:lincount} can also help inform the construction of linear codes with a small number of codewords in $S_\text{o}$: one such heuristic, for example, is to ensure that the dual code has many codewords that are \emph{not} present in $S_\text{o}$, thereby accumulating many words $\mathbf{s}$ at which the Fourier transform $\widehat{\mathds{1}_{S_{\text{o}}}}(\mathbf{s})$ is negative. 

Since we have that $S_\text{o} = \text{supp}_\text{o}\cup \text{supp}_\text{e}\cup \{0^n\}$, it is a simple task to directly compute the weight distribution of words in $S_\text{o}$. We hence skip the application of Theorem \ref{thm:wtcount} to this constraint.

==> sym.tex <==
\label{sec:sym}
The linear program $\mathsf{Del}(n,d;\mathcal{A})$ discussed in Section \ref{sec:sym}, for a fixed $\mathcal{A}\subseteq \mathbb{F}_2^n$, suffers from the drawback that the variables, which are precisely the values $(f(\mathbf{x}):\ \mathbf{x}\in \{0,1\}^n)$, are $2^n$ in number, i.e., exponentially large in the blocklength. The number of LP constraints, similarly, are exponentially large in $n$. It would therefore be of interest to check if the size of the linear program $\mathsf{Del}(n,d;\mathcal{A})$, which is the sum of the number of variables and the number of LP constraints, can be reduced, using symmetries present in the formulation.

Our exposition in this section on symmetrizing $\mathsf{Del}(n,d;\mathcal{A})$, follows that in \cite{linial1}. Let $S_n$ denote the symmetry group on $n$ elements, which is the set of all permutations $\sigma: [n]\to [n]$. Note that given a length-$n$ vector $\mathbf{x} = (x_1,\ldots,x_n)\in \{0,1\}^n$, a permutation $\sigma\in S_n$ acts on $\mathbf{x}$ as follows:
\[
\sigma \cdot \mathbf{x} = (x_{\sigma(1)},x_{\sigma(2)},\ldots,x_{\sigma(n)}).
\]
The permutation $\sigma$ also acts on functions $f: \{0,1\}^n\to \mathbb{R}$ via the mapping $(\sigma \circ f) (\mathbf{x})= f(\sigma\cdot \mathbf{x})$, for $\mathbf{x}\in \{0,1\}^n$. Now, given any set $\mathcal{A}\subseteq \mathbb{F}_2^n$, we define the ``symmetry group'' of the constraint represented by $\mathcal{A}$ to be the set of all permutations $\pi \in S_n$ that leave the indicator function $\mathds{1}_\mathcal{A}$ invariant. In other words, the symmetry group $G_\mathcal{A}$ of the constraint represented by $\mathcal{A}$ is the set of all permutations $\pi \in S_n$ such that $\mathds{1}_\mathcal{A} = \pi \circ \mathds{1}_\mathcal{A}$.

Given a group $G\subseteq S_n$ of permutations, which acts on the vectors $\mathbf{x}\in \{0,1\}^n$, we say that $\mathsf{Del}(n,d;\mathcal{A})$ is $G$-invariant, if for all $\sigma \in G$, it holds that if $f: \{0,1\}^n\to \mathbb{R}$ is a feasible solution to $\mathsf{Del}(n,d;\mathcal{A})$, then so is $\sigma \circ f$, with val$(f) = $ val$(\sigma\circ f)$. In what follows, we shall prove that $\mathsf{Del}(n,d;\mathcal{A})$ is, in fact, $G_\mathcal{A}$-invariant. Let $\pi\in G_\mathcal{A}$ be a permutation in the symmetry group of $\mathcal{A}$ and let $f$ be some feasible solution to $\mathsf{Del}(n,d;\mathcal{A})$.

\begin{itemize}
	\item[(D1)] It is clear that if $f(\mathbf{x})\geq 0$, then $f(\pi \cdot \mathbf{x})\geq 0$, for all $\mathbf{x}\in \{0,1\}^n$.
	\item[(D2)] The fact that if $\widehat{f}(\mathbf{s})\geq 0$, then it holds that $\widehat{\pi\circ f}(\mathbf{s})\geq 0$, for all $\mathbf{s}\geq 0$, follows from the simple lemma below:
	\begin{lemma}
		\label{lem:perm}
		For any function $f: \{0,1\}^n \to \mathbb{R}$ and for any permutation $\sigma \in S_n$, it holds that
		\[
		\widehat{\sigma \circ f}(\mathbf{s}) = (\sigma \circ \widehat{f})(\mathbf{s}), \quad \text{for all $\mathbf{s}\in \{0,1\}^n$}.
		\]
	\end{lemma}
\begin{proof}
	Observe that 
	\begin{align*}
		\widehat{\sigma \circ f}(\mathbf{s})&= \sum_{\mathbf{x}\in \{0,1\}^n} f(\sigma\cdot \mathbf{x})\cdot (-1)^{\mathbf{x}\cdot \mathbf{s}}\\
		&= \sum_{\mathbf{x}\in \{0,1\}^n} f(\sigma\cdot \mathbf{x})\cdot (-1)^{(\sigma\cdot\mathbf{x})\cdot (\sigma\cdot\mathbf{s})}\\
		&=\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x})\cdot (-1)^{\mathbf{x}\cdot (\sigma\cdot\mathbf{s})}
		=  (\sigma \circ \widehat{f})(\mathbf{s}).
	\end{align*}
\end{proof}
	\item[(D3)] Since any permutation in $G_\mathcal{A}$ also lies in $S_n$ and hence preserves the weights of vectors in $\{0,1\}^n$, it holds that $(\pi\circ f)(\mathbf{x}) = 0$, for all $\mathbf{x}\in \{0,1\}^n$ such that $1\leq w(\mathbf{x})\leq d-1$.
	\item[(D4)] This constraint is also satisfied by $\pi \circ f$, since $\pi(0^n) = 0^n$, for all $\pi\in G_\mathcal{A}$.
	\item[(D5)] Observe that for any $\pi\in G_\mathcal{A}$,
	\begin{align*}
		2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\pi\cdot \mathbf{x})&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\mathbf{z})\cdot \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{x}+\mathbf{z})\\
		&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{z})\cdot \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{x}+\pi\cdot \mathbf{z})\\
		&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{z})\cdot \mathds{1}_\mathcal{A}(\pi\cdot (\mathbf{x}+ \mathbf{z}))\\
		&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\mathbf{z})\cdot \mathds{1}_\mathcal{A}(\mathbf{x}+ \mathbf{z}) = 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}).
	\end{align*}
Hence, since for all $\mathbf{x}\in \{0,1\}^n$, we have that
\begin{align*}
\pi\circ f(\mathbf{x})&\leq 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\pi\cdot \mathbf{x})\\
&= 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}),
\end{align*}
we have that (D5) is also satisfied by $\pi\circ f$.
\item[(Obj$^\prime$)] It is clear that $\sum_{\mathbf{x}} f(\mathbf{x}) = \sum_{\mathbf{x}} f(\pi\cdot \mathbf{x})$, and hence that val$(f) = \text{val}(\pi\circ f)$.
\end{itemize}
From the preceding discussion, we see that given a feasible solution $f$ to $\mathsf{Del}(n,d;\mathcal{A})$, we can construct the function
\[
\overline{f}:= \frac{1}{|G_\mathcal{A}|}\sum_{\pi \in G_{\mathcal{A}}} \pi\circ f,
\]
such that $\overline{f}$ is also a feasible solution to the LP (by linearity), with val$(\overline{f}) = \text{val}(f)$. Observe, in addition, that $\overline{f}$ is such that $\pi\circ \overline{f} = \overline{f}$, for all $\pi\in G_\mathcal{A}$. Hence, it follows that in order to arrive at an optimal solution to $\mathsf{Del}(n,d;\mathcal{A})$, one can restrict oneself to searching among feasible solutions $f$ that are constant on each orbit $O$ in $\{0,1\}^n /G_\mathcal{A}$. Such functions $f$ can be expressed as
\begin{equation}
\label{eq:orbits}
f(\mathbf{x}) = \sum_{O\in \{0,1\}^n/G_\mathcal{A}} a_O\cdot \mathds{1}_O(\mathbf{x}),
\end{equation}
where $a_O \in \mathbb{R}$, for all $O\in \{0,1\}^n/G_\mathcal{A}$. Before we work on symmetrizing the constraints of $\mathsf{Del}(n,d;\mathcal{A})$, we introduce some notation. For an orbit $O\in \{0,1\}^n/G_\mathcal{A}$, we denote by $|O|$ the number of elements in the orbit and by $\mathbf{x}_O$ (or $\mathbf{s}_O$) a representative element of the orbit. Further, for a given element $\mathbf{x}\in \{0,1\}^n$, we define $O(\mathbf{x})$ to be the orbit in which $\mathbf{x}$ lies. We shall now formulate the constraints (D1)--(D5) and the objective function (Obj$^\prime$) in $\mathsf{Del}(n,d;\mathcal{A})$ based on \eqref{eq:orbits}.
\begin{itemize}
	\item[(D1$^\prime$)] The fact that $f(\mathbf{x})\geq 0$ for all $\mathbf{x}$ implies that $a_O\geq 0$, for all $O\in \{0,1\}^n/G_\mathcal{A}$.
	\item[(D2$^\prime$)] By the linearity of the Fourier transform operation, we obtain that 
	\[
	\widehat{f}(\mathbf{s}) = \sum_{O\in \{0,1\}^n/G_\mathcal{A}} a_O\cdot \widehat{\mathds{1}_O}(\mathbf{s})\geq 0,
	\]
	for all $\mathbf{s}\in \{0,1\}^n$.
	
	In fact, note that since $G_\mathcal{A} \subseteq S_n$, it can be argued using Lemma \ref{lem:perm} that the above inequality only needs to hold for orbit representatives $\mathbf{s}_O\in \{0,1\}^n$, of $O\in \{0,1\}^n/G_\mathcal{A}$. Indeed, we have that for any $\pi \in G_\mathcal{A}$,
	\begin{align*}
		\widehat{f}(\pi\cdot \mathbf{s}) &= \widehat{\pi \circ f}(\mathbf{s})\\
		&= f(\mathbf{s}), 
	\end{align*}
where the first equality holds by Lemma \ref{lem:perm} and the second holds since $\pi\circ f = f$, for functions $f$ as in \eqref{eq:orbits}.
	\item[(D3$^\prime$)] The constraint (D3) can be written as
	\[
	a_O = 0,\text{ for all $O$ such that $1\leq w(\mathbf{x}_O)\leq d-1$},
	\]
	where $\mathbf{x}_O\in \{0,1\}^n$ is a representative element of the orbit $O\in \{0,1\}^n/G_\mathcal{A}$.
	\item[(D4$^\prime$)] The constraint (D4) becomes
	\[
	a_{O(0^n)}\leq \text{val}(\mathsf{Del}(n,d)),
	\]
	where $O(0^n)$ is the orbit that contains the all-zeros word $0^n$.
	\item[(D5$^\prime$)] Similarly, the constraint (D5) reduces to
	\[
	a_O\leq 2^n\cdot(\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}_O),
	\]
	where, again, $\mathbf{x}_O$ is some representative element of the orbit $O\in \{0,1\}^n/G_\mathcal{A}$.
	\item[(Obj$^{\prime\prime}$)] From \eqref{eq:orbits}, we see that the new objective function simply becomes
	\[
	\underset{a_O\in \mathbb{R}}{\text{maximize}} \sum_{O\in \{0,1\}^n/G_\mathcal{A}} |O|\cdot a_O.
	\]
\end{itemize}
We call the symmetrized version of $\mathsf{Del}(n,d;\mathcal{A})$ as $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$, which is given below.
\begin{center}
	%	\begin{mybox}[colback=white, width = 0.75\linewidth]{$1,2$}
	%		This is my box.
	%	\end{mybox}
	\begin{tcolorbox}[title={\center $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$}, title filled = false, width = 0.65\linewidth]
		\begin{align}
			&\underset{\{a_O\in \mathbb{R}:\ O\in \{0,1\}^n/G_\mathcal{A}\}}{\text{maximize}} \ \ \sum_{O} |O|\cdot a_O \tag{Obj$^{\prime\prime}$}\\
			&\text{subject to:} \notag\\
			&\ \ a_O\geq 0, \forall\ O\in \{0,1\}^n/G_\mathcal{A}, \tag{D1$^\prime$}\\
			&\ \ \sum_{O\in \{0,1\}^n/G_\mathcal{A}} a_O\cdot \widehat{\mathds{1}_O}(\mathbf{s}_{\tilde{O}})\geq 0,\ \forall\ \text{orbit rep. } \mathbf{s}_{\tilde{O}}\in \{0,1\}^n, \tag{D2$^\prime$}\\
			&\ \ a_O = 0,\ \text{if $1\leq w(\mathbf{x}_O)\leq d-1$}, \tag{D3$^\prime$}\\
			&\ \ a_{O(0^n)}\leq \text{val}(\mathsf{Del}(n,d)), \tag{D4$^\prime$}\\
			&\ \ a_O\leq 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}_O),\ \forall\ O\in \{0,1\}^n/G_\mathcal{A}. \tag{D5$^\prime$}
		\end{align}
	\end{tcolorbox}
\end{center}
The preceding discussion can then be summarized as a theorem.
\begin{theorem}
	\label{thm:equiv}
	The LPs $\mathsf{Del}(n,d;\mathcal{A})$ and $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$ are equivalent in that
	\[
	\text{val}(\mathsf{Del}(n,d;\mathcal{A})) = \text{val}(\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})).
	\]
\end{theorem}

\begin{remark}
	All the above arguments remain valid if we use a subgroup $H$ of the symmetry group $G_\mathcal{A}$ as well. For the special case when $\mathcal{A} = \{0,1\}^n$, it holds that $G_\mathcal{A} = S_n$, and we then recover the more common version of Delsarte's LP that is $M_\text{LP}(n,d)$ in \cite{mrrw}. It is this version that we use for evaluating the right-hand side of constraints (D4) and (D4$^\prime$) in our numerical examples.
\end{remark}
Observe that in the symmetrized LP $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$, the number of variables is the number $N_\mathcal{A}$ of orbits $O\in \{0,1\}^n/G_\mathcal{A}$ and the number of constraints is at most $4N_\mathcal{A}+1$. Hence, if the constraint is such that the number of orbits $N_\mathcal{A}$ induced by its symmetry group is small (as a function of the blocklength $n$), then the size of the symmetrized LP is small. In the subsections that follow, we shall explicitly write down $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$, for select constraints (or sets $\mathcal{A}$), and provide numerical results obtained by running $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$ on those constraints.
\subsection{$2$-Charge Constraint}
\input{lp-2-charge.tex}
\subsection{Constant Subblock Composition Constraint}
\input{subblock.tex}
\subsection{Tail-Biting Constraints}
\input{tail-biting.tex}

==> tail-biting.tex <==
Next, we study upper bounds on the sizes of constrained codes for a given minimum distance, for a slightly stronger variant of the $(d,\infty)$-RLL constraint. In particular, we require that the constraint is satisfied across the boundary when the constrained sequence is cyclically wrapped around. We let $S^{\text{tail},d}$ denote this constraint that admits only those sequences $\mathbf{x}\in \{0,1\}^n$ such that $\mathbf{x}\in S^{d}$ and $\ell - s\leq n-d-1$, where $s \in [n]$ denotes the position of the first occurring $1$ in $\mathbf{x}$ and $\ell \in [n]$ denotes the position of the last occurring $1$. In the paragraphs that follow, we first identify the symmetry group of the more broad class of tail-biting constraints, to which $S^{\text{tail},d}$ also belongs.

Let a tail-biting constraint of interest be represented by a special set $\mathcal{A}$ of constrained sequences. In particular, $\mathcal{A}$ has the property that if a sequence $\mathbf{x}\in \mathcal{A}$, then $\pi^{\text{cyc},i}\cdot \mathbf{x}$ also lies in $\mathcal{A}$, where for $1\leq i\leq n$, $\pi^{\text{cyc},i}$ shifts each bit in $\mathbf{x}$ by $i$ bits to the left, wrapping around cyclically, if needed. More formally, $x_{\pi^{\text{cyc},i}(j)} = x_{\text{mod}(j+i,n)}$, for $1\leq j\leq n$. Clearly, we have that the symmetry group of the constraint $G_{\mathcal{A}}$ contains the cyclic group $C_n$, and it is hence possible to symmetrize $\mathsf{Del}(n,d;\mathcal{A})$ using $C_n$. The orbits $\boldsymbol{\alpha}$ thus are in one-one correspondence with (fixed) $2$-ary necklaces of length $n$, with turnovers prohibited (see pg. 18 in \cite{sedgewick} and sequence A000031 of \cite{oeis}). It is known that the number of such necklaces, and hence the number of orbits, $N_\text{cyc}(n)$, is such that $\lim_{n\to \infty} \frac{N_\text{cyc}(n)}{2^n/n} = 1$ (see \cite{stackexchange}); in other words, the sum of the number of variables and constraints in $\mathsf{Del}_{/G_\mathcal{A}}(n,d;\mathcal{A})$, is bounded above by $c\cdot\frac{2^n}{n}$, for some constant $c>0$, and large enough $n$. Thus, we obtain a slight reduction in the size of the LP as compared to $\mathsf{Del}(n,d;\mathcal{A})$, which had $2^n$ variables.

We then apply this symmetrization procedure to the tail-biting $(1,\infty)$-RLL constraint, $S^{\text{tail},1}$, which admits only binary sequences $\mathbf{x}\in \{0,1\}^n$ with no consecutive ones and which are such that $(x_1,x_n)\neq (1,1)$. Similar to the approach in the previous two subsections, we can set up a symmetrized LP $\mathsf{Del}_{/G_{S^{\text{tail},1}}}(n,d;S^{\text{tail},1})$, using the orbits of the cyclic group $C_n$.
Table \ref{tab:tail1} shows numerical evaluations of $\mathsf{Del}_{/G_{S^{\text{tail},1}}}(n,d;S^{\text{tail},1})$, when $n=13$, for varying values of $d$, and comparisons with the generalized sphere packing bound. Again, our LP provides tighter upper bounds than the generalized sphere packing bounds. Observe also that for certain values of minimum distance $d$, the optimal value of our LP coincides with the optimal value of the Delsarte LP $\mathsf{Del}(n,d)$.

\begin{table}[t!]
	\centering
	\begin{tabular}{||c || c || c || c ||} 
		\hline
		$d$ &$\mathsf{Del}_{/G_{S_{(1,\infty)}^\text{tail}}}(n,d;S_{(1,\infty)}^\text{tail})$& $\mathsf{GenSph}(n,d;S_{(1,\infty)}^\text{tail})$ & $\mathsf{Del}(n,d)$\\ [0.5ex] 
		\hline\hline
		$2$ & $480.676$ & $521$ & $4096$\\ 
		\hline
		$3$ & $350.055$ & $448.5$ & $512$\\ 
		\hline
		$4$ & $229.569$ & $448.5$ & $292.571$\\ 
		\hline
		$5$ & $64$ & $316.727$ & $64$\\ 
		\hline
		$6$ & $40$ & $316.727$ & $40$\\ 
		\hline
		$7$ & $8$ & $169$ & $8$\\ 
		\hline
		$8$ & $5.333$ & $169$ & $5.333$\\ 
		\hline
		$9$ & $3.333$ & $73.667$ & $3.333$\\ 
		\hline
	\end{tabular}
	\caption{Table of values of optimal values of the $\mathsf{Del}_{/G_{S^{\text{tail},1}}}(n,d;S^{\text{tail},1})$ LP, the generalized sphere packing bound LP $\mathsf{GenSph}(n,d;S^{\text{tail},1})$ in \cite{fazeli} and \cite{cullina}, and $\mathsf{Del}(n,d)$, for $n=13$, and varying values of $d$.}
	\label{tab:tail1}
\end{table}

==> valdel.tex <==
\section{Proof of Proposition III.1}
\begin{proof}
	Given the LP $\mathsf{Del}(n,d;\mathcal{A})$, defined by the objective function (Obj$^\prime$) and the constraints (D1)--(D5), we define the new LP $\overline{\mathsf{Del}}(n,d)$ with the same objective function (Obj$^\prime$) and using the constraints (D1)--(D4) alone (excluding constraint (D5)). Thus, $\overline{\mathsf{Del}}(n,d)$ is given by:
	\begin{align}
		&\underset{f:\ \{0,1\}^n\to \mathbb{R}}{\text{maximize}}\quad \sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x}) \tag{Obj$^\prime$}\\
		&\text{subject to:} \notag\\
		&\ \ f(\mathbf{x})\geq 0,\ \forall\ \mathbf{x}\in \{0,1\}^n, \tag{D1}\\
		&\ \ \widehat{f}(\mathbf{s})\geq 0,\ \forall\ \mathbf{s}\in \{0,1\}^n, \tag{D2}\\
		&\ \ f(\mathbf{x}) = 0,\ \text{if $1\leq w(\mathbf{x})\leq d-1$}, \tag{D3}\\
		&\ \ f(0^n)\leq \text{val}(\mathsf{Del}(n,d)), \tag{D4}
	\end{align}
	
	
	It is therefore clear that for any $\mathcal{A}\subseteq \{0,1\}^n$, it holds that val$(\mathsf{Del}(n,d;\mathcal{A}))\leq \text{val}(\overline{\mathsf{Del}}(n,d))$. We now claim that $\text{val}(\overline{\mathsf{Del}}(n,d))= (\text{val}({\mathsf{Del}}(n,d)))^2$. 
	
	First, we shall show that the inequality in constraint (D4) in $\overline{\mathsf{Del}}(n,d)$ can be replaced with an equality. To see this, suppose that $f$ were an optimal solution to $\overline{\mathsf{Del}}(n,d)$, with $f(0^n)<\text{val}(\mathsf{Del}(n,d))$. Let $c>0$ be such that $c\leq \text{val}(\mathsf{Del}(n,d))-f(0^n)$. We then construct the function $\overline{f}: \{0,1\}^n\to \mathbb{R}$ such that $\overline{f}(0^n) = f(0^n)+c$, and $\overline{f}(\mathbf{x}) = f(\mathbf{x})$, for $\mathbf{x}\neq 0^n$. It can then easily be verified that $\overline{f}$ satisfies constraints (D1), (D3) and (D4). Furthermore, $\overline{f}$ satisfies (D2) also, since by linearity of the Fourier transform, for any $\mathbf{s}\in \{0,1\}^n$, it holds that
	\begin{align*}
		\widehat{(\overline{f})}(\mathbf{s}) &= \widehat{f}(\mathbf{s})+c\cdot \widehat{\mathds{1}_{\{0^n\}}}(\mathbf{s})\\
		&= \widehat{f}(\mathbf{s})+\frac{c}{2^n}\geq 0.
	\end{align*}
Hence, $\overline{f}$ is a feasible solution to $\overline{\mathsf{Del}}(n,d)$, with val$(\overline{f}) = \sum\limits_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x})+c> \text{val}(f)$, which contradicts the optimality of $f$. Hence, any optimal solution to $\overline{\mathsf{Del}}(n,d)$ must be such that (D4) is satisfied with an equality, and we can thus replace the inequality in (D4) with an equality.

Now, in order to prove that $(\text{val}(\overline{\mathsf{Del}}(n,d)))^{1/2} = \text{val}({\mathsf{Del}}(n,d))$, it suffices to observe that any feasible solution $f$ of ${\mathsf{Del}}(n,d)$ yields a feasible solution $\text{val}(\mathsf{Del}(n,d))\cdot f$, to $\overline{\mathsf{Del}}(n,d)$ (with the inequality in (D4) changed to an equality). Likewise, any feasible solution $f$ of $\overline{\mathsf{Del}}(n,d)$ yields a feasible solution $\frac{f}{\text{val}(\mathsf{Del}(n,d))}$, to ${\mathsf{Del}}(n,d)$. Owing to this bijection, we obtain that $\text{val}(\overline{\mathsf{Del}}(n,d)) = \text{val}({\mathsf{Del}}(n,d))^2$.

Using the fact that val$(\mathsf{Del}(n,d;\mathcal{A}))\leq \text{val}(\overline{\mathsf{Del}}(n,d))$, we obtain the statement of the proposition.
\end{proof}

==> wtdistlin.tex <==
\label{sec:wtdistlin}
In this section, we briefly describe another useful computation that is facilitated by knowledge of the Fourier coefficients of the indicator function that a word belongs to a set of constrained sequences. Before we do so, we recall another property of Fourier transforms:
\begin{theorem}
	\label{thm:conv}
	Given functions $f,g:\{0,1\}^n\to \mathbb{R}$, the Fourier transform of $f\cdot g$ is the function $\widehat{f}\ostar \widehat{g}$, where
	\[
	\widehat{f}\ostar \widehat{g} (\mathbf{s}) := \sum_{\mathbf{z}\in \{0,1\}^n}\widehat{f}(\mathbf{z})\widehat{g}(\mathbf{z}+\mathbf{s}),\quad \mathbf{s}\in \{0,1\}^n.
	\]
\end{theorem}

The calculation we wish to perform puts together the theses of Theorems \ref{thm:lincount} and \ref{thm:wtcount}. In particular, we ask for the number of codewords of a linear code $\mathcal{C}$, which lie in a fixed set $\mathcal{A}$ and are of a given weight. We thus obtain Theorem \ref{thm:linwtcount}. For a given $\mathbf{v}\in \{0,1\}^n$, we use the notation $\mathbf{v}+\mathcal{C}$ to denote the coset of $\mathcal{C}$ to which $\mathbf{v}$ belongs. We let $a_{i,\mathcal{A}}(\mathcal{C})$ denote the number of constrained codewords of weight $i\in [0:n]$, which lie in the set $\mathcal{A}$ and in a linear code $\mathcal{C}$.
\begin{theorem}
	\label{thm:linwtcount}
	Given a linear code $\mathcal{C}$ of blocklength $n$, we have that
	\[
	a_{i,\mathcal{A}}(\mathcal{C}) = \frac{\left\lvert \mathcal{C}\right\rvert}{2^n} \sum_{j=0}^n K_i^{(n)}(j) \sum_{\mathbf{s}:\ w(\mathbf{s}) = j} \sum_{\mathbf{z}\in \mathbf{s}+\mathcal{C}^\perp} \widehat{\mathds{1}_{\mathcal{A}}} (\mathbf{z}).
	\]
\end{theorem}
\begin{proof}
	We observe that
	\begin{align*}
		a_{i,\mathcal{A}}(\mathcal{C}) &= \sum_{\mathbf{x}\in \{0,1\}^n} \mathds{1}_{W_i}(\mathbf{x})\cdot \mathds{1}_{\mathcal{A}}(\mathbf{x})\cdot \mathds{1}_{\mathcal{C}}(\mathbf{x})\\
		&{=} 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\mathds{1}_{W_i}}(\mathbf{s})\cdot \widehat{\mathds{1}_{\mathcal{A}}\cdot \mathds{1}_{\mathcal{C}}}(\mathbf{s}),
	\end{align*}
	where the last equality above uses Plancherel's Theorem (see Section \ref{sec:fourierprelim}). Further, by employing Theorem \ref{thm:conv} to expand the last equality, we get that
	\begin{align*}
		a_{i,\mathcal{A}}(\mathcal{C})&= 2^n\cdot \sum_{\mathbf{s}\in \{0,1\}^n} \widehat{\mathds{1}_{W_i}}(\mathbf{s})\cdot \left(\widehat{\mathds{1}_{\mathcal{A}}}\ostar \widehat{\mathds{1}_{\mathcal{C}}}\right)(\mathbf{s})\\
		&\stackrel{(a)}{=} \frac{\left\lvert \mathcal{C}\right\rvert}{2^n}\cdot \sum_{\mathbf{s}\in \{0,1\}^n} K_i^{(n)}(w(\mathbf{s}))\sum_{\mathbf{z}\in \{0,1\}^n} \widehat{\mathds{1}_{\mathcal{C}^\perp}}(\mathbf{z})\cdot \widehat{\mathds{1}_{\mathcal{A}}}(\mathbf{s}+\mathbf{z})\\
		&= \frac{\left\lvert \mathcal{C}\right\rvert}{2^n} \cdot  \sum_{j=0}^n K_i^{(n)}(j) \sum_{\mathbf{s}:\ w(\mathbf{s}) = j}\ \sum_{\mathbf{z}\in \mathbf{s}+\mathcal{C}^\perp} \widehat{\mathds{1}_{\mathcal{A}}} (\mathbf{z}),
	\end{align*}
	where equality (a) above uses the fact that $2^n\cdot  \widehat{\mathds{1}_{W_i}}(\mathbf{s}) = K_i^{(n)}(w(\mathbf{s}))$ and that $\widehat{\mathds{1}_{\mathcal{C}}}(\mathbf{s}) = \frac{\left\lvert \mathcal{C}\right\rvert}{2^n}\cdot \mathds{1}_{\mathcal{C}^\perp}(\mathbf{s})$ (see the proofs of Theorems \ref{thm:wtcount} and \ref{thm:lincount}).
\end{proof}

Theorem \ref{thm:linwtcount} could prove useful in the following context: consider the transmission of codewords of a linear code $\mathcal{C}$ over an input-constrained binary-input memoryless symmetric (BMS) channel, which admits only binary constrained sequences that lie in the set $\mathcal{A}$ as inputs. Suppose that the decoder being used is the maximum a-posteriori (MAP) (equivalently, the maximum likelihood (ML)) decoder of the linear code $\mathcal{C}$. By calculating the weight distribution of constrained codewords in a linear code $\mathcal{C}$ as above, it is possible to obtain an upper bound on the block error probability (via a union bounding argument), when the MAP decoder is used (see Chapter 1 of \cite{mct}).
